Coherent Control of Optogenetic Switching by Stimulated Depletion Quenching

Optogenetics is a revolutionary new field of biotechnology, achieving optical control over biological functions in living cells by genetically inserting light sensitive proteins into cellular signaling pathways. Applications of optogenetic switches are expanding rapidly, but the technique is hampered by spectral cross-talk: the broad absorption spectra of compatible biochemical chromophores limits the number of switches that can be independently controlled and restricts the dynamic range of each switch. In the present work we develop and implement a non-linear optical photoswitching capability, Stimulated Depletion Quenching (SDQ), is used to overcome spectral cross-talk by exploiting the molecules' unique dynamic response to ultrashort laser pulses. SDQ is employed to enhance the control of Cph8, a photo-reversible phytochrome based optogenetic switch designed to control gene expression in E. Coli bacteria. The Cph8 switch can not be fully converted to it's biologically inactive state ($P_{FR}$) by linear photos-witching, as spectral cross-talk causes a reverse photoswitching reaction to revert to it back to the active state ($P_{R}$). SDQ selectively halts this reverse reaction while allowing the forward reaction to proceed. The results of this proof of concept experiment lay the foundation for future experiments that will use optimal pulse shaping to further enhance control of Cph8 and enable simultaneous, multiplexed control of multiple optogenetic switches.

==> ch-OG/App_BG.tex <==
\appendix
\section{Background: The Cph8 Optogenetic Switch}\label{Sec:OG:BGCph8}
Cph8 is a recently developed phytochrome based optogenetic switch designed to control gene expression in E. Coli bacteria \cite{Levskaya2005}. Naturally occurring phytochromes are light sensing proteins in plants, algae, cyanobacteria, and other micro-organisms that harness light as an energy source \cite{Neff2000, Vierstra2000}. These organisms rely on phytochromes to respond to daily and seasonal changes to the light environment. In plants phytochromes control seed development and growth \cite{Franklin2010, Chen2011}, while in algae and cyanobacteria they act as primitive vision sensors to steer toward or away from light during phototaxis \cite{PHP:PHP1481,Garcia2000}. Phytochromes use the photo-isomerization of a covalently attached open-chain tetrapyrrole (bilin) chromophore to reversibly convert between two states in response to light. The chromophore cycles between a dark-stable, red-absorbing $P_R$ state and a meta-stable, far-red-absorbing $P_{FR}$ state, functioning as a molecular switch to regulate numerous responses to light intensity, color, duration, and direction \cite{Smith1995}.

Structurally, phytochromes all share a conserved, modular architecture consisting of an N-terminal photo-sensory module and a C-terminal signal-output module, shown in Figure~\ref{Fig:OG:PhytArch}. The photo-sensory module is made up of three domains: PAS (Per/ARNT/Sim), GAF (cGMP phosphodiesterase/adenylate cyclase/FhlA), and PHY (phytochrome-specific) \cite{Psakis2011}. The bilin chromophore is covalently anchored to a conserved cysteine residue in the GAF domain; and the PAS and GAF domains surround the chromophore, forming the protective binding pocket that isolates the molecule from the surrounding environment, enabling coherent optical interactions within the ``hot, wet, and noisy conditions inside a living cell''\cite{Lloyd2011}. The PHY domain detects the isomerization of the chromophore and mediates the translation of the nanometer scale isomerization of the chromophore into the large scale re-orientation of the remaining phytochrome that can be registered by the cellular signaling architecture and affect biological functions.
\begin{figure}[htb]
	\centering
	\includegraphics[width=.7\linewidth]{ch-OG/Figs/Intro/Fig_PhytArchS}
	\caption[Phytochrome Architecture]{The Cph1 protein complex, divided into the conserved architecture of the canonical phytochrome, which makes up the Photo-Sensory Module of Cph8. The PAS and GAF domains anchor and form the binding pocket around the chromophore phycocyanobilin (PCB). The PHY domain detects the state of the chromophore and passes the information to the Signal Output Module on the other side of the cell membrane, which transforms the information into a cellular signal pathway initiating biological function. (Adapted from \cite{Essen2008})}
	\label{Fig:OG:PhytArch}
\end{figure}
The phytochrome photo-sensory module has a simple modular architecture that shows up naturally in a wide range of species and can be artificially implemented in a number of cell types: including mammalian and bacterial cells \cite{Auldridge2011}. Phytochrome based optogenetic controls seem to be possible in any organism containing the appropriate chromophore (either natively generated, as in many plant and mammalian cells, or exogenously created in bacteria and other cell types) \cite{Burgie2014Rev}. This adaptability and natural wide utility across many cell types will be important for the expansion of phytochrome based switches and the possible multiplexed optical control of multiple switches, which will be expanded upon in Section~\ref{Sec:OG:Conclusions}.

Cph8 is an artificial fusion protein that combines a phytochrome light-sensing domain with a Two Component Signaling system (TCS) native to E. coli.
The phytochrome light sensor is Cph1, originally from the cyanobacterium \emph{Synechocystis PCC6803}, which utilizes phycocyanobilin (PCB) as a chromophore \cite{Gambetta2001}.
The E. Coli TCS is EnvZ, whose normal function is sensing changes in the osmolarity of the surrounding environment \cite{vanAlphen1977}. Under red light illumination the light-sensing domain is excited from the dark stable $P_R$ state to the $P_{FR}$ state, sending a stimulus to the downstream signal output module of the EnvZ half of the Cph8 switch. When activated by stimuli from the sensor domain, EnvZ selectively phosphorylates the OmpR response regulator, a small mobile enzyme in the cell cytoplasm that promotes gene transcription when phosphorylated \cite{Gao2008}. When the switch returns to the $P_R$ state, either by far-red light illuminated or by slow, automatic dark reversion, the EnvZ output module de-phosphorylates the P-OmpR response regulator, inhibiting transcription. The specific gene sequence that OmpR associates with can be engineered into the system. For example, cells have been programmed to generate pigments \cite{Tabor2011} or fluorescent proteins \cite{Schmidl2014} in response to optical switching under exposure to light, so as to provide measurable evidence of the switching function.  A schematic of this TCS system is shown in Figure~\ref{Fig:OG:Cph8Tabor}(a), along with a representative measurement of the light activated production of GFP protein in Cph8 expressing bacteria (b). In Figure~\ref{Fig:OG:Cph8Tabor}(b) the non-zero signal under 650 nm illumination shows the effect of spectral cross-talk (i.e., the system is incapable of being turned off under normal illumination).

\begin{figure}
	\centering
	\includegraphics[width=.7\linewidth]{ch-OG/Figs/Intro/Fig_Cph8Tabor}
	\caption[Cph8 Switching Function]{(adapted from Ref~\cite{Schmidl2014})(a) Schematic of the Cph8-OmpR light-switchable Two Component Sensing system. The sample is exposed to Far-red (740 nm) and red (650 nm) LEDs to initiate switching. Red light partially switches Cph8 from the $P_R$ to $P_{FR}$ form. Far-red light or extended periods of dark conditions revert Cph8 $P_{FR}$ to $P_R$. (b) Mean sfGFP fluorescence of populations of E. coli carrying Cph8-OmpR and illuminated with saturated red and far-red light. Due to spectral cross-talk the GFP signal cannot be fully turned off.}\label{Fig:OG:Cph8Tabor}
\end{figure}

Figure~\ref{Fig:OG:Cph8Spec} (an expansion of Figure~\ref{OG:FullExpConcept}(b))shows the absorption spectra of the Cph8 sample after exposure to red and far-red light until saturation of the photoswitching transition. After far-red exposure the switch has fully converted to the $P_R$ state, as this state does not appreciably absorb at wavelengths longer than 720 nm and there is no forward ($P_R\rightarrow P_{FR}$) photoswitching reaction.
\begin{figure}
	\centering
	\includegraphics{ch-OG/Figs/Intro/Fig_Cph8Spec}
	\caption[Cph8 Absorption]{Absorption spectra of the Cph8 sample.
		The red line shows the spectrum of the pure \pr state, obtained by maintaining the sample under saturated far-red illumination ($\lambda=725$ nm). The purple line is associated with a sample in the photoequilibrium mixed state of 65\% \pr and 35\% \pfr, obtained by maintaining the sample under saturated red illumination ($\lambda=650$ nm). From the difference of these spectra we can extract the pure \pfr spectrum, shown by the dashed blue line. The ultimate goal of this work is clean switching to this projected pure $P_{FR}$ state.}
	\label{Fig:OG:Cph8Spec}
\end{figure}
However, due to overlap of the $P_R$ and $P_{FR}$ absorption spectra at shorter wavelengths, the red light exposure activates both the forward and reverse ($P_{FR}\rightarrow P_R$) photoswitching reactions, and the sample does not fully convert to the $P_{FR}$ state. This photoequilibrium is defined by the ratio of the forward and reverse reaction rates at the excitation wavelength. At 650 nm this equilibrium is 65\% $P_{FR}$, 35\% $P_R$ \cite{Lamparter2002}. This photoequilibrium greatly limits the functional application of these switches (as with the majority of optically sensitive biological molecules) due to the broad overlapping absorption spectra of naturally evolved chromophores.
Stated another way, this spectral cross-talk limits the dynamic range of the switch: the ratio of the final cellular functional output under activating and de-activating light inputs is restricted by preventing the switch from being fully converted to the $P_{FR}$ state.



The source of the spectral cross-talk is the overlap in the absorption spectra of the two chromophore states in the light-sensing module. To increase the dynamic range of the switch we must uncouple the optical interaction with the \pr state (which activates the forward photoswitching reaction) from the optical interaction with the \pfr state (which activates the reverse reaction). We have demonstrated theoretically \cite{ Li2002, Turinici2004, Li2005} and experimentally \cite{ Roth2009, Petersen2010, Rondi2011, Roslund2011, Rondi2012} that even molecules with spectra that are nearly functionally identical can be differentially excited by exploiting their unique, coherent excited state dynamics using ultrashort tailored pulsed light sources. To independently optically address the two states of the Cph8 protein complex we must investigate the photo-isomerization dynamics of the PCB chromophore molecule.


\section{Background: Chromophore Dynamics}\label{Sec:OG:BGPCBDyn}

The chromophore in the photo-sensory module of Cph8, phycocyanobilin (PCB), is made up of four pyrrole rings labeled A-D in Figure~\ref{Fig:OG:PhyPCB}(b) (an expansion of Figure~\ref{OG:FullExpConcept}(a)) in an open configuration joined by conjugated methine bridges. The A-ring of the chromophore is covalently bound to the GAF domain at the Cys259 residue \cite{Essen2008,Lamparter2001}(as shown in Figure~\ref{Fig:OG:PhyPCB}(a)). This domain surrounds the chromophore, forming the binding pocket, which constrains the structure of the chromophore and influences its spectral response and dynamics, while isolating it from environmental disturbances that would destroy the effectiveness of the photo-isomerization reaction. The structure of the chromophore and the surrounding binding pocket shown in Figure~\ref{Fig:OG:PhyPCB}(a) is based on x-ray crystallographic analysis of the Cph1 phytochrome in the \pr state \cite{Essen2008}. The D-ring of the chromophore is less constrained than the rest of the molecule, giving it the freedom of movement to flip between two conformational states.
The planar $ZZZ_{ssa}$ isomer conformation corresponds to the red-light absorbing $P_R$ state. A rotation of the D-ring about the  $C_{15}$=$C_{16}$ carbon bridge flips it out of the plane of the other three pyrroles converting the chromophore to the $ZZE_{ssa}$ conformation associated with the far-red-light absorbing \pfr state. Here $Z(usammen) \& E(ntgegen)$ and $s(yn) \& a(nti)$ refer to the symmetry of the double and single bonds, respectively, of the \emph{C5}, \emph{C10}, and \emph{C15} carbons in the methine bridges joining the four pyrrole rings of the bilin chromophore.
In the $P_{FR}$ state, interaction with the Tyr176 residue of the GAF domain (also labeled in Figure~\ref{Fig:OG:PhyPCB}(a)) affects down stream changes in the rest of the phytochrome, converting the nanometer scale isomerization of the chromophore into a large-scale re-distribution of neighboring domains producing a signaling pathway that can influence cellular function.
The optical characteristics of the chromophore are very sensitive to the binding pocket: mutation of alleles in the PAS and GAF domains of the phytochrome can prevent photoswitching or shift the absorption spectrum by up to 30 nm \cite{Shcherbakova2016}. In spite of these shifts, the change in the central wavelength is always smaller than the broad, overlapping absorption spectrum characteristic of the bilin chromophores, meaning it is still susceptible to spectral cross-talk. However, it should be noted that while not sufficient to distinguish species by linear absorption, these subtle shifts to the chromophore binding pocket should provide an ultimate basis to exploit pulse shaping for optimal dynamic discrimination (ODD) of multiple similar switches (see Section~\ref{Sec:OG:Conclusions}).

\begin{figure}
	\centering
	\includegraphics[width=.8\linewidth]{ch-OG/Figs/Intro/Fig_PhyPCB}
	\caption[Chromophore Structure and Isomerization]{(a) (Adapted from \cite{Essen2008}) Ribbon representation structure of the binding pocket in the GAF domain of the Cph1 photo-sensory module. The PCB chromophore is covalently attached to the GAF domain at C-259. The tyrosine residue Y176 is believed to help stabilize the $P_{FR}$ state and is important in the photoswitching reaction. (b) PCB Chromophore in the $P_R$ and $P_{FR}$ states. The $C_{14}\!\!-\!\!C_{15}$=$C_{16}$ methine bridge linking the C-ring and D-ring is highlighted. The two states partially interconvert with red light (650 nm), and concomitantly under far-red light (720 nm) or dark-reversion. }\label{Fig:OG:PhyPCB}
\end{figure}

As discussed above, the absorption of the $P_{FR}$ state extends to longer wavelengths than $P_R$, yielding near complete ($>$97\%) conversion from the $P_{FR}$ to the $P_R$ state (the reverse reaction) under constant far-red excitation. The opposite reaction is challenging due to spectral cross-talk: the red light excitation is absorbed by both the $P_R$ and $P_{FR}$ states.
Since we cannot solve the problem of spectral cross-talk by altering the absorption spectra, we must turn to an alternate set of optical interactions to find suitable controls to differentiate the states. While the ground state absorption of the $P_R$ and $P_{FR}$ states are similar and overlapping, the excited state dynamics are very different and open a new avenue for controlling the chromophores and differentiating the two states. Thus, we seek to exploit the distinct dynamics of the forward and reverse photo-isomerization reaction to halt the reverse reaction while minimizing the impact on the forward reaction.

The photo-isomerization of the PCB chromophore in both directions is initiated by photo-excitation of the molecule, immediately followed by very rapid coherent vibronic relaxation on the excited state surface \cite{Heyne2002}. This sequence is then followed by a portion of the excited molecules transitioning to a transient intermediate product state beginning the isomerization. The remaining excited state population returns to its respective initial ground state. In the forward isomerization reaction ($P_R\rightarrow P_{FR}$) this intermediate is LUMI-R; in the reverse ($P_{FR}\rightarrow P_R$) the intermediate is LUMI-F \cite{Bischoff2000,Bischoff2001}. These two transient intermediate species are unique to the forward and reverse reaction, respectively, and the subsequent relaxations progress along distinct, separate reaction coordinates.  The LUMI-R and LUMI-F transient intermediate products persist for several nanoseconds and trigger a series of large scale conformational reorganizations of the protein residues in the downstream domains to complete the photoswitching transformation between the $P_R$ and $P_{FR}$ states of the full Cph8 switch. The names ``\pr'' and ``\pfr'' are used to refer to the red-light and far-red-light absorbing states, respectively, of the PCB chromophore, the phytochrome light-sensing module, and the overall Cph8 switch depending on context.

The initial coherent steps of the ultrafast photo-isomerization are not as well understood as the slower domain reorganizations associated with the latter steps of the switching. It is generally agreed that the isomerization in both directions is initiated when the PCB chromophore absorbs a photon of light, exciting an electron from the $\pi$-conjugated system primarily localized on the C and D pyrrole rings and the methine bridge that joins them. This promotes an electron to the anti-bonding $\pi$* orbital, weakening the double bonding character of the $C_{15}$-$C_{16}$ carbon atoms in the bridge (labeled on the chromophores in Figure~\ref{Fig:OG:PhyPCB}(b)), enabling rotation of the outer D ring and inter-conversion between the $P_R$ state and the $P_{FR}$ state, and vice versa, by way of non-shared transient intermediates. \cite{Bischoff1998, Bischoff2001, Heyne2002}. It is here that the forward ($P_R\rightarrow P_{FR}$) and reverse ($P_{FR}\rightarrow P_R$) photo-isomerization reactions start to differ and also where the disagreements about the earliest dynamics of the excited state relaxation begin.
In particular, the early stage dynamics of the initial excited state relaxation and isomerization steps of the Cph1 phytochrome have been studied using numerous ultrafast electronic \cite{Heyne2002, Fitzpatrick2012, Kim2012} and vibrational \cite{Dasgupta2009, vanWilderen2009, vanThor2007, Yang2012} transient spectroscopies, often arriving at different and sometimes even contradictory conclusions.
In all reported studies, analysis of time-resolved spectra reveal complex multi-exponential excited-state relaxation dynamics, but there are different interpretations of these measurements. The extent of the isomerization reaction occurring on the excited state and the homogeneity of the ground state population are the principle areas of disagreement.
There are two schools of thought with regard to ground state population:
(1) there is an ensemble of ground state sub-populations that each undergo distinct single-exponential dynamics after excitation (the “inhomogeneous perspective”), and
(2) there is a single uniform ground state population and the complex, non-exponential excited state dynamics are due to multiple vibronic resonances at a conical intersection (the “homogeneous perspective”).

Each perspective is supported by a number of experimental studies using a variety of measurement techniques. Resonant Raman intensity analysis \cite{Spillane2009} and hybrid quantum mechanics/molecular mechanics (QM/MM) simulations \cite{Mroginski2010}support a homogeneous \pr state that undergoes multi-phasic excited state dynamics. Solid-state NMR resolved two distinct ground state \pr sub-populations: one structure consistent with the known crystal structure and a second interpreted as having a modified charge distribution and hydrogen bond network \cite{Song2011}. Some pump-dump-probe (PDP) studies find evidence of a homogeneous ground state in $P_R$ \cite{vanWilderen2009, Fitzpatrick2012}, while other PDP experiments observe a heterogeneous ground state in Cph1 \cite{Kim20140618,Kim2013,Kim2012}and in a related phytochrome \cite{Chang2013}. There is currently no consensus as to the exact nature of the ultrafast dynamics of the photo-isomerization.
The results of the most recently published experiments characterizing the forward and reverse photo-isomerization reactions are summarized below.

The forward photo-isomerization of $P_R$ to $P_{FR}$ of the Cph1 phytochrome has been characterized by the Larsen group from UC Davis \cite{Kim20140417}. The study consists of a combination of temperature-dependent and excitation-wavelength-dependent static and ultrafast transient absorption measurements. Using a global analysis of the combined measurements they resolve five distinct ground state sub-populations (Pr1, ..., Pr5) co-existing at thermal equilibrium, each undergoing single-exponential dynamics through separate excited and intermediate states. The sub-populations can be grouped into two distinct categories: the fast-decaying photo-active populations (Pr1 and Pr5) and the slow-decaying fluorescent populations (Pr3-Pr5). The exponential lifetimes associated with each sub-population at room temperature are summarized in Figure~\ref{Fig:OG:Larsen}. The time scale of the forward isomerization is given by the formation of LUMI-R in 61 picoseconds.


\begin{figure}
	\centering
	\includegraphics[width=5in]{ch-OG/Figs/Intro/Fig_Larsen}
	\caption[Forward photoswitching dynamics reveal Heterogeneous $P_R$ Ground State]{(adapted from~\cite{Kim20140417}) Measurements of forward photoswitching dynamics reveal heterogeneous ground state sub-populations. The photoswitching population (${P_r2}$ above) forms the LUMI-R intermediate isomerization product with a time constant of 61 ps.}\label{Fig:OG:Larsen}
\end{figure}

The reverse ($P_{FR}\rightarrow P_R$) photo-reaction has been less thoroughly studied due to the transient nature of the $P_{FR}$ state and inability to fully remove the confounding $P_R$ state. In a collaboration between the Heyne group at the Freie Universitat Berlin and the Mathies group at UC Berkeley, a combination of Femtosecond Stimulated Raman Spectroscopy (FSRS) and polarization-resolved transient IR spectroscopy was used to map the initial steps of the reverse photo-isomerization reaction from the $P_{FR}$ state of the Cph1 phytochrome \cite{Yang2016}. Researchers detected the extremely rapid sub-picosecond development of the LUMI-F intermediate product. This observation is supported by direct measurement of the orientation of the chromophore D-ring by the femtosecond resolved polarization anisotropy of the $C_{19}$=O vibrational absorption (a good indicator of the orientation of the ring) as shown in Figure~\ref{Fig:OG:HeyneMathies}(a-c). The FSRS measurement of the $C_{15}$=$C_{16}$ stretch in Figure~\ref{Fig:OG:HeyneMathies}(d) shows the shift to lower wavenumber of the stretching vibration, which reflects a reduction in the vibrational force constant after relaxation from the FC region. The inset of Figure~\ref{Fig:OG:HeyneMathies}(d) shows the ground-state recovery dynamics of the 1607 $cm^{-1}$ bleach feature fit to a bi-exponential decay curve with time constants of $t_1$=(300$\pm$50) fs and $t_2$=(6$\pm$3) ps, representing a $\approx$70\% loss of the excited population within a picosecond of excitation; in agreement with the timescale of the ring flip given by the IR measurement.


\begin{figure}
	\centering
	\includegraphics[width=.95\linewidth]{ch-OG/Figs/Intro/Fig_HeyneMathies}
	\caption[Reverse photoswitching reaction involves complex excited state dynamics]{(adapted from~\cite{Yang2016}) (a-b) Measurements and analysis of the polarization resolved transient IR absorption and (d) FSRS measurements of the reverse photo-isomerization of PCB in Cph1 phytochrome. (a) Ultrafast transient absorption of the ground state $\nu (C_{19}$=$O)$ and $\nu (C_{19}$=$O)$* vibrational modes on the electronic ground and excited state energy surfaces. Black dots in (a) represent IR probe polarization parallel to the visible excitation, while red circles represent perpendicular probe polarization. The vertical blue bars illustrate that the difference between the two polarized absorption signals remains fixed in the ground state, but rapidly changes in the excited state. This provides direct measurement of the rotation of the ($C_{19}$=O)* vibrational mode and, by extension, the D-ring of the chromophore.
		(b) The polarization anisotropy quantifies the difference between the two polarized absorption signals and is a measure of the angle between the transition dipole moments of the electronic excitation and the vibrational mode. The time varying anisotropy of the excited state ($C_{19}$=O)* mode is strong evidence of rotation of the D-ring in the excited state with a time constant of 0.7 ps.
		(c) Charts of the shift in peak FSRS frequency of the excited state $C_{15}$=$C_{16}$ stretch associated with a weakening of the bond order after excitation. The inset shows the ground-state bleach dynamics for the $C_{15}$=$C_{16}$ stretch, exhibiting bi-exponential recovery of the ground state over two time domains: a fast 300 fs recovery and a slower 6 ps recovery. These figures are a condensed selection of many measurements from reference~\cite{Yang2016} which support the conclusion of sub-picosecond coherent isomerization in the reverse ($P_{FR}\rightarrow P_R$) photoswitching reaction.}\label{Fig:OG:HeyneMathies}
\end{figure}

Analysis of multiple vibrational modes on the chromophore and the direct measure of the ultrafast change in the polarization anisotropy of the $C_{19}$=O on the D-ring support sub-picosecond isomerization of the PCB chromophore to the LUMI-F transient photo-product. The ultrafast structural change in the bilin chromophore may indicate formation of the first intermediate state on the excited state potential surface, and is accelerated by a non-bonding “methyl-methyl clash” of the outer methyl groups on the C-ring and D-ring in the $P_{FR}$ ground state. A representation of the excited state dynamics on a 2-D potential energy surface is shown in Figure~\ref{Fig:OG:HMConInt}. The relaxation from the initial Frank-Condon excitation point ($P_{fr}^*$  in Figure~\ref{Fig:OG:HMConInt}) occurs in 300 fs, at which point the molecule either relaxes back to the $P_{FR}$ ground state or remains on the excited surface, depending on whether its D-ring has initiated rotation. Those chromophores remaining in the excited state continue to rotate until reaching the conical intersection with the LUMI-F photo-product surface over the next 700 fs. The conical intersection mediates the rapid generation of the LUMI-F photo-product.
\begin{figure}
	\centering
	\includegraphics[width=.8\linewidth]{ch-OG/Figs/Intro/Fig_HeyneMathiesConInt}
	\caption{(adapted from~\cite{Yang2016}) (a) Sketch of the multi-dimensional potential energy surface representative of the isomerization reaction, which is shown on the right (b). Non-bonding interactions between the methyl groups on the C and D rings (indicated with green ``\textcolor[rgb]{0,0.6,0}{\textbf{)(}}'' in (b)) place a strain on the \pfr ground state which enhances the speed of the reverse isomerization once initiated by absorption of a photon. The important vibrations that are part of the reaction coordinate in the multi-dimensional PES are depicted on the axes in (a). The two-step mechanism of the isomerization process is depicted by the black and red trajectories. The conical intersection, denoted by a grey square, enables very fast generation of the LUMI-F photoproduct and $P_{FR}$ ground state.}\label{Fig:OG:HMConInt}
\end{figure}


These studies inform our understanding of the Cph8 switch and guide the development of the experiment reported in this chapter. While the exact details of the excited state dynamics are neither fully understood nor agreed upon, this situation does not hinder our ability to conduct experiments exploring a pathway to the control of the optogenetic switches.
The ability to distinguish the two states of the Cph8 switch does not require exact knowledge of the coherent excited state dynamics of the molecule, only the ability to interact with the system while the excited state coherent dynamics are ongoing.
Built on the essence of the background experiments reported here, a kinetic-based model may be constructed using the generalized switching picture captured in Figure~\ref{OG:FullExpConcept}(c) (Section~\ref{Sec:OG:REMSim}). We will see that, there are inherent features of the photo-physics in the latter figure (i.e., the stability of the two switch states, and the irreversibility of the switching dynamics once initiated) that are amenable to identifying the per-exposure iterative map for the transfer of population between the switch states.
The existence of this iterative map is more important than a detailed quantitatively accurate model.
The experiments in this work (Section~\ref{Sec:OG:SDQExp}) will identify the map from the laboratory data, and then use the properties of the iterative map to calculate the effective transfer for the $P_R \rightarrow P_{FR}$ photoswitching reaction.
Importantly, the conclusions drawn from these initial experiments should apply to further advanced studies, including pulse-shaping assisted multiplexed optimal dynamic discrimination of multiple similar optogenetic switches.





==> ch-OG/Sec_Intro-Sims.tex <==
%\singlespacing

\section{Introduction and Background}\label{Sec:OG:IntroBG}


\subsection{Introduction}\label{Sec:OG:Introduction}

%\doublespacing

The variety and complexity of tasks performed by living cells is astonishing: they harvest and refine chemicals from their environment \cite{Albertsch2}, synthesize complex chemicals in response to demand \cite{Gething1992}, respond to changes in their environments in ways that mirror logic and memory \cite{HOPFIELD199453}, self-replicate and multiply under globally limited constraints \cite{AlbertsEssentials,Ardissone2016}, and work together - communicating and combining to form multi-cellular tissues \cite{Albertsch19}.
A cell accomplishes all these tasks by measuring an array of internal and external environmental conditions using various sensor protein complexes and performing a specific biological function in response, as dictated by a set of instructions in its genetic code. In this way, cells behave as functional machines, performing actions in direct response to stimuli.
Recently, biologists have developed the capability to genetically engineer cells, supplanting the natural sensors with light sensitive proteins. These engineered proteins enable the activation or suppression of specific cellular functions with optical signals, turning a piece of the naturally developed sensing-response system into an externally accessible ``control panel''.
This approach, called \emph{optogenetics} \cite{Deisseroth2011, Pastrana2011}, enables the precise and reversible control of specific biological processes in living cells by external optical stimuli to systematically perturb the system and observe its response\cite{Fenno2011}.

Currently available optogenetic tools can control a range of biological processes including ion channel activation
%(enabling its primary application as a high fidelity neuromodulation technique
(enabling high fidelity neuromodulation \cite{Zemelman2002, Boyden2005, XiangLi2005}), organism mobilization \cite{Wen2012, Leifer2011, LeiferPhD2011} and behavior \cite{Montgomery2015, Gunaydin20141535, Husson2013},
protein synthesis in cells \cite{Olson2012,Tabor2011},
%
% Optogenetic control is typically mediated by
gene expression or inhibition \cite{Shimizu-Sato2002, Konermann2013, Cao2013, Tyszkiewicz2008},
protein localization at specific cell sites \cite{Levskaya2009, Toettcher20131422, Toettcher2011, Toettcher2011409, Leung02092008},
or sequestration of active proteins away from their site of reaction \cite{Lee2014, Yang01082013}.
Optical techniques can be very appealing for the control and monitoring of biological systems, with many advantages over physical or chemical/pharmacological activation.
Light is a noninvasive tool that interacts strongly with specific biologically relevant molecules and can be applied with high spatial and temporal resolution.
Precise activation signals can be encoded into many controllable parameters of the optical signal, including the light's intensity, frequency spectrum, phase structure, and the duration or temporal pattern of the exposure. Moreover, optical stimuli can be rapidly halted, in contrast to diffusionally controlled chemicals.

In spite of these favorable aspects, the practical implementation of optogenetics is prevented from reaching its fullest potential by spectral cross-talk: the overlapping optical responses of the switches.
Most chromophores, the molecules within the optogenetic switch that absorb light, have broad, featureless absorption spectra, which limits the number of switches that can be independently addressed by linear photo-excitation.
More problematic is that for many switches even the absorption spectrum of the activated and de-activated states overlap, preventing the switch from being completely converted from one state to the other.
This inability to distinguish the two states of the switch limits the accessible dynamic range of the system and fidelity of control.

The capability now exists to overcome the spectral cross-talk: it has been shown that even molecules with nearly identical static absorption spectra can exhibit unique dynamical responses to ultrashort laser pulses \cite{Courvoisier2006}.
These distinguishable dynamics can be accentuated by a set of optimal optical control pulses to distinguish similar molecular species, this technique is known as Optimal Dynamic Discrimination (ODD) \cite{Li2002, Turinici2004, Li2005,Roth2009, Petersen2010, Rondi2011, Roslund2011, Rondi2012,Goun2016}.
By interacting with the time-dependent non-linear optical response of a molecule, rather than just the static absorption spectrum, we increase the number of control parameters that can be varied to search for orthogonal optical controls that are not restricted by the same spectral cross-talk as the linear optical responses.
A suitable set of orthogonal optical controls should be capable of separating the optical responses of several similar optogenetic switches that would be extremely difficult to independently address by conventional linear photo-excitation.
The ultimate goal of this research is the simultaneous (multiplexed) control of multiple optogenetic switches over their maximum dynamic range, thereby independently and simultaneously controlling a large number of cellular functions.
In the present work we take the first step toward the goal of multiplexed control of multiple optogenetic switches by developing a model to simulate the optical interaction between such pulses and a simplified optogenetic switch. Results with this model indicate that the dynamic range of the switch can be enhanced beyond the linear photoequilibrium limit imposed by spectral cross-talk.


The simplified optogenetic switch modeled in this paper is based on Cph8, a phytochrome based red/far-red sensing optogenetic switch developed for controlling gene expression in E. Coli bacteria \cite{Levskaya2005, Tabor2009,Tabor2011}.
More detailed information about the Cph8 switch and the dynamics of its internal chromophore \emph{phycocyanobilin} (PCB) will be provided in Appendices \ref{Sec:OG:BGCph8} and \ref{Sec:OG:BGPCBDyn}. 
%To summarize briefly:
Cph8 is an artificial ``fusion'' protein, a synthesis of the light sensing domains of the Cph1 protein originally found in Cyanobacteria with the Histidine-Kinase Two-Component Switch (TCS) signalling domains of EnvZ, a protein native to E. Coli that is associated with gene transcription \cite{Schmidl2014}.
The chromophore in the Cph8 switch, phycocyanobilin (PCB), converts between two states by photo-isomerization, as shown in Figure~\ref{OG:FullExpConcept}(a).
The gene-expressing ``On'' state absorbs red light and is called \pr, while the biologically inactive ``Off'' state is called \pfr because its absorption spectrum is shifted to longer wavelengths in the far-red. The absorption spectra of these two states is shown in Figure~\ref{OG:FullExpConcept}(b).
\begin{figure}
  \centering
  \includegraphics[width=5.9in]{ch-OG/Figs/Intro/ExpConcept_2}
  \caption[Overview of Experimental Concept]{
  	Overview of the Controlled Optogenetics experimental concept: (a) Photoswitching of Cph8 is initiated by photo-isomerization of the PCB chromophore between an active state $(P_{R})$ and an in-active state $(P_{FR})$. The \pfr state can be completely removed with far-red light, however spectral cross-talk prevents complete removal of the \pr state. 
  	(b) Absorption spectra of a sample of Cph8 in the pure 100\% \pr state, the photoequilibrium mixed state of 65\% $P_{FR}$/35\% $P_{R}$, and the pure 100\% \pfr state that we aim to reach by Stimulated Depletion Quenching (SDQ) enhancement.
  	(c)\emph{SDQ Concept:} The Cph8 sample in a mix of \pr and \pfr states is exposed to ultrashort Excitation and Depletion pulses, separated by a delay $\uptau$. Both states are excited and undergo dissimilar coherent ultrafast excited state dynamics along a chromophore isomerization coordinate to either the transient product states (LUMI-R and LUMI-F) or back to their initial ground states (grey arrows). The transient products more slowly transform the remaining protein domains downstream of the chromophore, completing the photoswitching reaction.
  	Precision timing of the depletion pulse permits the selective transfer of a larger portion of the $P_{FR}$* molecules back to the $P_{FR}$ ground state (i.e., quenched molecules no longer follow grey dashed arrows) compared to the same process for $P_R$*, thereby quenching the reverse reaction more than the forward. This process shifts the equilibrium of the photoswitching reaction toward \pfr, increasing the dynamic range of the Cph8 switch.
}
  \label{OG:FullExpConcept}
\end{figure}
The Cph8 switch can be fully converted from the \pfr state to the \pr state by continuous illumination with far-red light ($\lambda \geq$ 720 nm), this is described as the ``reverse'' photo-isomerization reaction.
Deactivation of the switch, converting from the \pr state to the \pfr state, is described as the ``forward'' photo-isomerization reaction, and due to the overlapping absorption spectra of the two states there is no wavelength of light that will initiate the forward photo-isomerization reaction without also initiating the reverse reaction.
The simultaneous photo-reaction between the two states under red-illumination comes to photoequilibrium with a maximum \pfr population of $\sim65\%$ (\pr$\sim35\%$). The absorption spectrum of a sample in this equilibrium mixed state is also shown in Figure~\ref{OG:FullExpConcept}(b).
%\tcb{The goal of this research is to push past this linear photoequilibrium threshold and achieve nearer to 100\% \pfr.}
Using ultrashort laser light pulses we will exploit the unique dynamic optical responses of the \pr and \pfr states to selectively ``quench'' the reverse photoswitching reaction, $P_{FR} \rightarrow P_R$, by stimulated depletion, shifting the photoequilibrium to increase the dynamic range of the switch.




A schematic of the proposed \emph{Stimulated Depletion Quenching (SDQ)} mechanism is shown in Figure~\ref{OG:FullExpConcept}(c), and will be more fully explained in Section~\ref{Sec:OG:ExpDesc}.
To summarize, the actuation of the Cph8 switch is initiated when the PCB chromophore absorbs a red or far-red photon.
%and an electron is excited from the highest conjugated $\pi$-orbital of the molecule to an anti-bonding $\pi$*-orbital. This process weakens the bond order of the methine bridge joining the outer C and D rings of the chromophore, resulting in molecular isomerization by rotation of the D-ring, producing an irreversible cascade of down-stream protein domain reorganizations converting that single electronic excitation into the activation of a cellular signaling pathway.
This excitation weakens the bond order of the methine bridge joining the outer C and D rings of PCB, resulting in molecular isomerization by rotation of the D-ring, producing an irreversible cascade of down-stream protein domain reorganizations converting that single electronic excitation into the actuation of a cellular signaling pathway.
Due to spectral cross-talk of the \pr and \pfr states both are excited by photons of red light, it is not possible to prevent these unwanted electronic excitations of the \pfr state of the PCB chromophore.
% with conventional direct radiative absorption.
% and the switch can never be fully turned off by conventional light exposure. an equilibrium concentration of activated switches always persists.
%One potential means of eliminating spectral cross-talk would entail re-engineering the photo-sensory domain to alter the absorption spectrum of the chromophores. Accomplishing this without diminishing the effectiveness of the signaling pathway is challenging, and has not been accomplished at the current time. Furthermore, even if the states of an individual switch could be distinguished, any attempts to utilize multiple optogenetic switches or to use them in concert with fluorescent reporters would quickly run into the same problem of spectral cross-talk due to the inherent limited fidelity and range of the single parameter of excitation/emission wavelength.
However, it \emph{is} possible to prevent the switching of the remainder of the Cph8 protein complex and subsequent activation of the cellular signaling pathways by de-exciting the chromophore before the larger protein ``notices'' that it has been triggered.
After the excitation to the $P_{R}^\ast$ or $P_{FR}^\ast$ state there is a brief interval of time before the chromophore begins isomerization. During this interval the molecule can be returned to its initial state by stimulated depletion, making it appear as though no absorption had occurred and quenching the photoswitching reaction.
%To maintain the optical control of the system in this approach, the excited electron would be transferred to the ground state by stimulated emission.
Further, to facilitate this capability, there should be sufficient differences in the excited state dynamics and stimulated emission spectra of the two forms of the chromophore to preferentially depopulate the $P_{FR}$* excited state over that of the $P_R$* excited state, allowing the forward reaction to proceed while quenching the reverse reaction.
This selective quenching shifts the photoequilibrium of the simultaneous forward and reverse photoswitching reactions, thereby increasing the maximum attainable $P_{FR}$ population.
The total photoswitching reaction can be represented by a simple linear transformation map for an incremental $P_R \rightarrow P_{FR}$ step per laser interaction; upon repeated iteration of the mapping transform (i.e., repeated laser exposure) the full transition of large populations of the Cph8 switch from the \pr to the \pfr state can be accomplished. The components of the transformation map can be calculated from a small number of measurements of the system, enabling us to rapidly calculate the photoequilibrium population and the enhancement of the dynamic range accessible by the Cph8 switch brought on by the SDQ mechanism.

The experimental research described here is a feasibility study of this proposed SDQ mechanism, aiming to demonstrate control of the photo-isomerization reaction in the Cph8 optogenetic switch by achieving greater stimulated depletion quenching of the reverse photoswitching reaction compared to the forward reaction by harnessing the unique dynamics of the two photo-isomerization pathways.
This work has a limited goal, but represents an important first step toward the ultimate goals of achieving maximal dynamic range control of a single optogenetic switch and simultaneous independent control of multiple optogenetic switches in living cells by multiplexed, optimal non-linear photoswitching.


%The chapter is organized as follows.
The remainder of this introduction section contains additional background information on the Cph8 phytochrome based switch (Section~\ref{Sec:OG:BGCph8}), the photo-isomerization of the PCB chromophore associated with Cph8 (Section~\ref{Sec:OG:BGPCBDyn}), and a more detailed description of the proposed SDQ technique (Section~\ref{Sec:OG:ExpDesc}).
Section~\ref{Sec:OG:REMSim} describes a model for simulations assessing the feasibility of the experiment and exploring the significant reduced parameter space to determine an effective range of experimental parameters.
Section~\ref{Sec:OG:SDQExp} presents the experimental controlled photoswitching of the Cph8 system and the procedure for data processing and analysis of the resulting measurements.
These processed data are further analyzed and results are presented in Section~\ref{Sec:OG:Results}, followed by a discussion of the current results and recommended future experimental directions in Section~\ref{Sec:OG:Conclusions}.


%Photoswitching from the ``ON state'' to the ``OFF state'' (the so-called ``forward reaction'') is often achieved by the same wavelengths of light as the ``reverse reaction" (``OFF'' to ``ON'') due to the overlapping absorption spectra of the states.

%\section{Background}\label{Sec:OG:BG}
\subsection{Description of the SDQ Mechanism}\label{Sec:OG:ExpDesc}

%\begin{figure}
%  \centering
%  \includegraphics[width=.65\linewidth]{ch-OG/Figs/ExpConcept_Schem}
%  \caption[Diagram of Experimental Concept]{Diagram of SDQ Experimental Concept: The Cph8 sample is exposed to the ultrashort Excitation and Depletion pulses, separated by $\uptau_{Delay}$. Both initial states of the switch are excited and the molecules undergo ultrafast relaxation toward the branching conical intersection to either the transient product states (LUMI-R and LUMI-F) or back to the initial ground states. There is good spectral overlap of the depletion pulse with the $P_{FR}$* excited state depletion spectrum (red arrow connects surfaces) and poor overlap with the $P_{R}$* depletion spectrum (red arrow too short to connect surfaces). A barrier on the $P_R$* excited surface slows the forward reaction. The combination of spectral overlap and timing permit the depletion pulse to coherently and selectively drive a larger portion of the $P_{FR}$* excited molecules back to $P_{FR}$ ground state, quenching the reverse reaction more than the forward. (the quenched molecule no longer follows the path of the grey dashed arrows)}\label{Fig:OG:ExpConcept}
%\end{figure}

In this experiment selective stimulated emission is employed to coherently transfer PCB chromophores initially excited to the $P_{FR}$* state back to the \pfr ground state before isomerization can occur, while simultaneously allowing chromophores initially excited to the $P_{R}$* state to persist and undergo photoswitching to the $P_{FR}$ state.
The concept of this SDQ mechanism is represented in the diagram in Figure~\ref{OG:FullExpConcept}(c).
The sample is exposed to two ultrashort laser pulses: an excitation pulse and a depletion pulse.
The spectrum of the excitation pulse overlaps with the absorption spectra of both the $P_{R}$ and $P_{FR}$ states of the PCB chromophore. Exciting the molecule with the ultrashort pulse creates corresponding coherent wave packets from superpositions of vibrational levels on the electronic excited state surfaces of both forms of the chromophore.
These wave packets undergo dissimilar coherent dynamics as they relax from their initial Frank-Condon excitation states toward a coherent vibronic transition through a conical intersection either back to their initial ground state or to a transient intermediate photo-product state.
Before the molecules complete these dynamics, a second pulse arrives after a short, controlled delay ($\uptau_{Delay}$).
This depletion pulse has a central wavelength set to overlap more favorably with the stimulated emission spectrum of the $P_{FR}$* state than the $P_{R}$* state.
The combination of spectral overlap and timing permit the depletion pulse to selectively drive a larger portion of the $P_{FR}$* excited molecules back to the $P_{FR}$ ground state, preferentially slowing the reverse photo-isomerization reaction while allowing the forward reaction to continue transferring some portion of the \pr population to the \pfr state.
Those molecules remaining in either of the excited states after the depletion pulse continue their unperturbed dynamics, either isomerizing to the transient photo-product state or returning to their initial ground state.
%The relative final populations of the Cph8 switch in each state after being exposed to the pulsed excitation and depletion sequence are measured by absorption spectroscopy.


In this work, the excitation and depletion pulse parameters will be varied to determine the wavelengths, powers, pulse durations, and delay timings which selectively deplete the $P_{FR}$* level most effectively, quenching the reverse reaction while minimally hindering the forward reaction.
This exploration of the experimental control parameter space aims to be a feasibility study for the proposed mechanism, identifying a path through the vast, unexplored control landscape toward a region amenable to effective control of the photoswitching reaction, thereby laying the foundation for more sophisticated optimal control experiments on optogenetic switches in the future.




==> ch-OG/Sec_REMSim.tex <==
%\singlespacing

\section{\nohyphens{SDQ Feasibility Assessed by Rate Equation Model Simulations}}\label{Sec:OG:REMSim}
%Control of photoswitching by Stimulated Depletion Quenching

%\doublespacing


We perform simulations using a Rate Equation Model (REM) to qualitatively assess how a system, with optical characteristics and ultrafast dynamics corresponding to the Cph8 switch, responds to ultrashort-pulsed laser excitation and depletion under experimentally reproducible conditions.
The SDQ mechanism is an iterative control scheme, shifting the equilibrium condition of the simultaneous forward and reverse photoswitching reactions such that over repeated laser exposures the system gradually moves toward the desired final product distribution in many small steps.
To this end, we first model how the system responds to a single excitation-depletion pulse sequence in Section~\ref{Sec:OG:REMSingle}. These single exposure simulations generate a set of \emph{Characteristic Coefficients}, which describe the photoswitching reaction products independent of the initial state conditions, defined exclusively by the laser exposure condition.
In Section~\ref{Sec:OG:REMMulti}, the products of the simulated single exposure photoswitching reaction are used to generate an Optical Transformation Matrix (OTM), which is a linear transformation from the initial to the final state population.
% defined solely by the characteristics of the laser pulse sequence.
The OTM can be used to easily simulate repeated exposures of a system, generating an iterative mapping from the initial state to any final state of the system within the Maximal Dynamic Range (MDR) accessible by the associated laser exposure defined by the particular control parameter set.
We apply this iterative mapping to show how repeated exposures allow the $P_{FR}$ state to gradually reach a higher photoequilibrium enhanced by SDQ.
%\textcolor[rgb]{0.00,0.00,1.00}{The iterative transfer of population between the \pr and \pfr states over many exposures is an important and unique characteristic of the photoswitching reaction, as it defines an iterative mapping of the initial state to any final state within the dynamic range of the switch defined solely by the illumination of the sample. This iterative mapping is a function of the laser control parameters, and not the state of the system...}
Once the mechanics of the simulation are explained, in Section~\ref{Sec:OG:REMSurvey} we present a collection of results showing the functional dependence of the photo-reaction on the laser control parameters and locate the region of the parameter space that most effectively enhances the photoswitching dynamic range.
These simulations are designed to provide a basis to guide and understand the experiments of Section~\ref{Sec:OG:SDQExp}, and the model predictions for the SDQ enhancement will be compared to the measured results in Section~\ref{Sec:OG:Results}.
While the simplicity of the model precludes total quantitative agreement, the simulations and experimental results share the most common feature of an iterative map driven transfer mechanism.
The Matlab code used in these simulations will be maintained on the servers of the Rabitz group and can be provided upon request.


\subsection{Simulation of Dual-Pulsed Excitation-Depletion Photoswitching}\label{Sec:OG:REMSingle}

A schematic of the model system is shown in Figure~\ref{Fig:OG:UFModel}. In comparison to Figure~\ref{OG:FullExpConcept}(c) or Figure~\ref{Fig:OG:HMConInt}(a), the multi-dimensional potential energy surfaces of the $P_{R}$, $P_{R}$*,$P_{FR}$ and $P_{FR}$* states have each been collapsed to two discrete levels representing each surface, and a pair of levels represent the transient intermediate products LUMI-R=LR5 and LUMI-F=LF5, totaling ten levels.
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{ch-OG/Figs/REM/Fig_UFModel_labeled}
  \caption[Rate Equation Model Schematic]{Schematic of relevant states and transitions for simulation of the photoswitching reaction by REM. Solid arrows represent optically coupled transitions between the electronic ground and excited states while dashed lines are spontaneous relaxations between states. The transitions are labeled by their rate coefficients: the constant values of the spontaneous transitions are collected in Table~\ref{Tab:OG:kijs} while the variable coefficients of the optically coupled transitions are functions of the laser controls as described by Eq~\ref{OG:RateMod:SpecRateConst} in the text. The intermediate states LUMI-R (LR5) and LUMI-F (LF5) do not interact, transferring their entire accumulated population to the ground level of the opposite chromophore state at the end of the photoswitching reaction.}
  \label{Fig:OG:UFModel}
\end{figure}
Rather than describing discrete states separated by single-valued energy differences, the levels should be viewed as representing manifolds of molecular states, and the optical responses and associated dynamics of the levels are defined by experimentally measured absorption and emission spectra and state lifetimes associated with time resolved measurements, as discussed further below.
The model supports excitation to a Frank-Condon point and subsequent relaxation in the electronic excited state followed by either isomerization to the intermediate product state or transition to a hot ground state by spontaneous relaxation or stimulated emission.
The populations of the intermediate states, LUMI-R and LUMI-F, do not cross or interact (i.e., the intermediate transition states during the forward isomerization from $P_{R}$ to $P_{FR}$ are not shared with the transient states of the reverse reaction); once isomerization begins it will continue unabated.
The branching ratio of the isomerization/spontaneous emission pathways is dictated by the relative transition rate constants, which are based on excited state level lifetimes from experimental measurements \cite{Kim20140417, Yang2016}.
%\footnote{Put in the following descriptions or just cite? ``... current literature: the $P_{R}$ rate constants were measured by Dual-Excitation pump-probe transient absorption spectroscopy \cite{ Kim20140417 } while the $P_{FR}$ rate constants were obtained by combined analysis of polarization resolved transient IR spectroscopy and femtosecond Stimulated Raman \cite{Yang2016 }''}
%\tcg{With further information about the excited state dynamics a more physically complete model incorporating a degree of coherence could be simulated. The results of the present rate equation model can be thought of as a conservative picture of what can be achieved by the SDQ mechanism, as it does not allow for pulse shaping of the excitation and depletion pulses to exploit coherence effects in the excited state dynamics. }
The rate constants associated with the spontaneous transitions in Figure~\ref{Fig:OG:UFModel} are collected in Table~\ref{Tab:OG:kijs}.
Using these parameters, the model reproduces the expected behavior under single-pulse excitation. In particular, when exposed to continuous red illumination ($\lambda=650$ nm) the switch reaches a mixed state equilibrium of $P_{FR}/P_{R}\simeq 65\%/35\%$ and fully resets to $>99\%P_{R}$ under continuous far-red illumination ($\lambda >725$ nm).

\begin{table}[b]
\centering
\small
  \begin{tabular}{ @{}m{1.2in}@{} @{}m{1.2in}@{} @{}m{1.15in}@{} @{}m{1.152in}@{} @{}m{1.3in}@{} }
	\toprule
	\thead{ Electronic \\ Relaxation } & \thead{ Fast \\ Isomerization } & \multicolumn{2}{c}{\thead{Vibrational Relaxation}} & \thead{Slow \\ Isomerization} \\
	\midrule
	$k_{3,4}^{R} = \nicefrac{1}{26 ps}$ & $k_{3,5}^{R} = \nicefrac{1}{61 ps}$ & $k_{2,3}^{R} = \nicefrac{1}{0.15 ps}$ & $k_{4,1}^{R} = \nicefrac{1}{0.15 ps}$ & $k_{LR5-FR1}=\nicefrac{1}{10^9 ps}$\\
    $k_{3,4}^{FR} = \nicefrac{1}{0.30 ps}$ & $k_{3,5}^{FR} = \nicefrac{1}{1.50 ps}$ & $k_{2,3}^{FR} = \nicefrac{1}{0.05 ps}$ & $k_{4,1}^{FR} = \nicefrac{1}{0.05 ps}$ & $k_{LF5\rightarrow R1} = 	\nicefrac{1}{10^9 ps}$\\
    \bottomrule
    \end{tabular}
  \caption{Static rate coefficients of REM. Coefficients are expressed as inverse lifetimes associated with values from the literature \cite{ Kim20140417, Yang2016}. }\label{Tab:OG:kijs}
\end{table}

Because details of the structure and coherent dynamics of the chromophore molecules in the phytochrome switching systems are still not fully understood, the coherent energy-time coupling properties of the molecule and the laser pulses are not contained in this kinetic model.
The high-dimensional, vibronically coupled potential energy surfaces are simplified to a reduced number of levels associated with the integrated spectral response of the molecule and linked by spontaneous incoherent transitions.
The pulsed lasers are characterized under the slowly varying envelope (SVE) approximation: the temporal dynamics of the pulse serves only to scale the fixed spectral intensity distribution, leaving the coherent spectral phase and fast oscillating component of the complex-valued electric field out of the calculation.
These simplifications allow us to simulate the system without making further assumptions about characteristics of the excited state dynamics that are not conclusively accepted.
The next generation of improved modeling, incorporating better knowledge of the system's structure and dynamics from future measurements
%and \tcb{built on an estimate of the molecular Hamiltonian of the constrained chromophore system, }
would allow for a degree of coherence in the dynamics of the system using an appropriate quantum master equation (i.e., the Lindblad equation) to simulate the evolution of the sample population distribution.
While details associated with the coherent dynamics of the molecule are not present, the rate equation model offers qualitative insight into \emph{how} the rapid kinetics of the photo-isomerization reaction impacts the practicability of the SDQ method. In this way, the rate equation model can be thought of as a worst-case limit of the capability of the SDQ method as it does not exploit coherence.

Starting with the measured reference absorbance spectra of the Cph8 protein in the $P_{R}$ and $P_{FR}$ states, we can simulate or approximate the remaining features of the model.
%with a few reasonable assumptions and approximations.
The reference absorbance spectra are shown in Figure~\ref{Fig:OG:SimSpecs}, scaled to the peak molecular absorption cross-section. The absorption spectra in the literature~\cite{Lamparter2002} are reported as the molar attenuation coefficient, but the calculations require the molecular cross-section; the conversion between the two is simply: \(\sigma(\lambda)=\nicefrac{10^3ln(10)}{N_{Av}}\times\varepsilon(\lambda)\).
The peak molar attenuation coefficient of the \pr state is $\varepsilon_R (650\ nm)=85$ $(mM cm)\up{-1}$ and the corresponding value for the peak of the \pfr state is $\varepsilon_{FR} (705nm)=65.9$ $(mM cm)\up{-1}$, resulting in a peak absorption cross-section of $\sigma_R(650)=3.24\times10^{-16} cm^2$ and $\sigma_{FR}(705)=2.51\times10^{-16} cm^2$ for the \pr and \pfr states, respectively.
There is no measurement of the stimulated emission cross-section for the chromophore; however, we can represent the emission spectrum by reflecting the absorption spectrum across the zero phonon line \cite{MukamelNLO}. Comparing the absorption/emission spectra of similar species, notably the iRFP fluorescent protein species developed by mutation of the Cph1 photo-sensory module \cite{Zhu2015}, this symmetry is common and the assumption is reasonable. These simulated emission spectra are also plotted in Figure~\ref{Fig:OG:SimSpecs} using dashed lines.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{ch-OG/Figs/REM/Fig_SimSpecs}
  \caption[Spectra used in Rate Equation Model]{Absorption (solid lines) and stimulated Emission (dashed  lines) spectra of Cph8 in the $P_{R}$ state (red curves peaking at 665 nm and 725 nm, respectively) and the $P_{FR}$ state (black curves peaking at 710 nm and 770nm, respectively). Also plotted are spectra representing an excitation pulse centered at 625 nm and two different depletion pulses centered at 775 nm and 835 nm (orange, light red, and dark red shaded areas, respectively).} \label{Fig:OG:SimSpecs}
\end{figure}

We define the excitation and depletion pulses in terms of their real-valued spectral intensity, described here by a scaled Gaussian distribution. For the pulse \emph{p} = (\emph{Ex.} (excitation) or \emph{Dp.} (depletion)) centered at wavelength $\lambda_0^p$ and with full width at half max of $\Delta \lambda_p$, the real spectral intensity is:

\begin{equation}\label{Eq:OG:SpecIntensity}
  I_{p}(\lambda; \lambda_0^p, \Delta \lambda_p, \langle P_p \rangle,d_p)=\left(\dfrac{4\langle P_p \rangle}{\pi\cdot d_p^2}\right)\left(\dfrac{2\sqrt{ln2}}{\Delta \lambda_p \sqrt{\pi}}\right)e^{-({2\sqrt{ln2}\cdot (\lambda -\lambda_0^p)}/{\Delta \lambda_p})^2}
\end{equation}

\noindent The spectral distribution function is scaled by the average power $\langle P_{p} \rangle$ (in units of Watts) and beam waist diameter $d_{p}$ (in units of cm) to give the spectral intensity in (\nicefrac{W}{cm\up2}). The ``beam diameter'' is defined in these simulated pulses to describe the intensity in terms of experimentally measured and controlled parameters. The spectra of the excitation and depletion pulses are plotted with the molecular absorption and emission spectra in Figure~\ref{Fig:OG:SimSpecs} for an excitation pulse centered at 625 nm with width 30 nm and two separate depletion pulses with width 10 nm, one centered at 775 nm and the other at 835 nm.

The temporal intensity of the pulse is defined by a normalized Gaussian function with variable delay $t_0^{p}$ and an adjustable pulse width $\Delta t_p$:

\begin{equation}\label{Eq:OG:TempIntensity}
  I_{pulse}(t; t_0^p, \Delta t_p,)=\left(\dfrac{2\sqrt{ln2}}{\Delta t_p \sqrt{\pi}}\right) e^{-\left({2\sqrt{ln2}\cdot (t-t_0^p)}/{\Delta t_p}\right)^2}
\end{equation}

\noindent As stated above, the model simulates the pulsed laser under the slowly varying envelope (SVE) approximation, the temporal intensity envelope is defined independently from the fixed spectral intensity distribution, rather than using a complex phase term in the field amplitude to stretch the broad bandwidth, ultrashort pulse beyond its transform-limited duration.
This approximation is acceptable where the spectral frequency bandwidth of the pulse is much smaller than the central frequency: $\Delta \omega / \omega_0 <<1$.
For the spectral bandwidths and pulse durations used in these simulations we are straining the acceptable usage of the SVE approximation (for a Gaussian spectrum 30 nm wide centered at 625 nm the ratio of bandwidth to central frequency is 0.048).
%, and it might be more technically correct to represent the pulses with the frequency-time coupled representation
However, because the model only incorporates
%the real-valued intensities of the pulses and
the integrated spectral overlap of the lasers and the total spectral response of the molecules (which are much broader than the laser bandwidth) a time-varying spectral distribution would have little effect on the calculated rate coefficients while greatly complicating the calculations. In subsequent models, where different laser pulse shapes will excite distinct excited vibronic population distributions with distinct dynamics, it will be necessary and useful to represent the laser pulse by a spectral-temporal coupled field and incorporate coherent aspects of the molecular dynamics.

With the reference absorption and emission spectra of the simulated Cph8 molecule and the modeled excitation and depletion pulses, we can calculate the dynamic rate constants for the optical transitions in the molecule and simulate the time dependent populations of each level for both the $P_{R}$ and $P_{FR}$ states. The initial conditions are defined, with each state having a fraction of the total chromophore population in its lowest ground state:
\begin{align}\label{OG:RateMod:IC}
  [P_R]_{init} &= R1_0 \\
  [P_{FR}]_{init} &= FR1_0=(1-R1_0)
\end{align}
\noindent where $0 \leq R1_0 \leq 1$. The time dependent populations of the levels of the $P_{R}$ and $P_{FR}$ states are given by the solution to a set of coupled first order differential rate equations (see Figure~\ref{Fig:OG:UFModel} for reference to the notation).
The five coupled differential equations describing the populations of the five levels associated with the \pr state (R1-LR5) are shown below in Equations~\ref{ER1}-\ref{ER5}. The five \pfr levels (FR1-LF5) are described by five more equations of the same form in Equations~\ref{EFR1}-\ref{EFR5}, exchanging appropriate rate constants and populations for the $P_{FR}$ levels.
The \pr and \pfr states are coupled by the transfer from level LR5 to FR1 (eqs. \ref{ER5},\ref{EFR1}) and LF5 to R1 (eqs. \ref{EFR5},\ref{ER1}).
The rate equations for the $P_R$ associated levels are:
\begin{subequations}
\label{EREM}
\begin{align}
\begin{split}
  \dfrac{d(R1(t))}{dt} ={}& [K_{1,2}^{R,Ex}(t)+K_{1,2}^{R,Dep}(t)]\cdot (R2(t)-R1(t))\\
  &\quad +(k_{4,1}^R\cdot R4(t))+(k_{LF5\rightarrow R1}\cdot LF5(t))
  \label{ER1}
  \end{split}\\
\begin{split}
  \dfrac{d(R2(t))}{dt} ={}& [K_{1,2}^{R,Ex}(t)+K_{1,2}^{R,Dep}(t)]\cdot (R1(t)-R2(t))\\
  &\quad -(k_{2,3}^R\cdot R2(t))
  \label{ER2}
  \end{split}\\
\begin{split}
  \dfrac{d(R3(t))}{dt} ={}& [K_{3,4}^{R,Ex}(t)+K_{3,4}^{R,Dep}(t)] (R4(t)-R3(t))\\
  &\quad +(k_{2,3}^R\cdot R2(t))-(k_{3,4}^R\cdot R3(t))-(k_{3,5}^R\cdot R3(t))
  \label{ER3}
  \end{split}\\
\begin{split}
  \dfrac{d(R4(t))}{dt} ={}& [K_{3,4}^{R,Ex}(t)+K_{3,4}^{R,Dep}(t)]\cdot (R3(t)-R4(t))\\
  &\quad +(k_{3,4}^R\cdot R3(t))-(k_{4,1}^R\cdot R4(t))
  \label{ER4}
  \end{split}\\
\dfrac{d(LR5(t))}{dt} ={}& (k_{3,5}^R\cdot R3(t))-(k_{LR5\rightarrow FR1} \cdot LR5(t)),
\label{ER5}
\end{align}
\end{subequations}

\noindent while the rate equations for the $P_{FR}$ associated levels are:
\begin{subequations}
\label{EREM_FR}
\begin{align}
\begin{split}
  \dfrac{d(FR1(t))}{dt} ={}& [K_{1,2}^{FR,Ex}(t)+K_{1,2}^{FR,Dep}(t)]\cdot (FR2(t)-FR1(t))\\
  &\quad +(k_{4,1}^FR\cdot FR4(t))+(k_{LR5\rightarrow FR1}\cdot LR5(t))
  \label{EFR1}
  \end{split}\\
\begin{split}
  \dfrac{d(FR2(t))}{dt} ={}& [K_{1,2}^{FR,Ex}(t)+K_{1,2}^{FR,Dep}(t)]\cdot (FR1(t)-FR2(t))\\
  &\quad -(k_{2,3}^{FR}\cdot FR2(t))
  \label{EFR2}
  \end{split}\\
\begin{split}
  \dfrac{d(FR3(t))}{dt} ={}& [K_{3,4}^{FR,Ex}(t)+K_{3,4}^{FR,Dep}(t)] (FR4(t)-FR3(t))\\
  &\quad +(k_{2,3}^{FR}\cdot FR2(t))-(k_{3,4}^{FR}\cdot FR3(t))-(k_{3,5}^{FR}\cdot FR3(t))
  \label{EFR3}
  \end{split}\\
\begin{split}
  \dfrac{d(FR4(t))}{dt} ={}& [K_{3,4}^{FR,Ex}(t)+K_{3,4}^{FR,Dep}(t)]\cdot (FR3(t)-FR4(t))\\
  &\quad +(k_{3,4}^{FR}\cdot FR3(t))-(k_{4,1}^{FR}\cdot FR4(t))
  \label{EFR4}
  \end{split}\\
\dfrac{d(LF5(t))}{dt} ={}& (k_{3,5}^{FR}\cdot FR3(t))-(k_{LF5\rightarrow R1} \cdot LF5(t)).
\label{EFR5}
\end{align}
\end{subequations}

In the rate equations above, the molecule moves from level \emph{i} to level \emph{j} via \emph{spontaneous transitions}, governed by rate constants $k_{i,j}^S$
or by \emph{optically coupled transitions} governed by coefficients $K_{i,j}^{S,pulse}(t)$ (where the $S$=($R$ or $FR$) denotes the association with the $P_{R}$ or $P_{FR}$ initial state).
The transition coefficients have units $ps^{-1}$.
As stated earlier, the spontaneous transition coefficients are related to measured excited state dynamic lifetimes from the literature, and are collected in Table~\ref{Tab:OG:kijs}. The vibrational relaxation rate constants of both states ($k_{2,3}^S$ and $k_{4,1}^S$) are very high, associated with the very short vibrational relaxation lifetimes.
As such, levels 2 and 4 have fleeting populations serving primarily as intermediaries to levels 1 and 3.

The optically coupled transition rate coefficients ($K_{i,j}^{S,pulse}(t)$) are ``dynamic'', and vary with the intensity of the pulse temporal envelope. These coefficients are calculated individually for the excitation and depletion pulses. For the chromophore population in state \emph{S} = (\emph{R} or \emph{FR}), interacting with \emph{pulse(p)}=(\emph{Ex}(Excitation) or \emph{Dep}(Depletion)) the time dependent rate of transition from level \emph{i} to \emph{j} is given by :
\begin{equation}\label{OG:RateMod:SpecRateConst}
  K_{i,j}^{S,pulse}(t)= I_{pulse}(t;t_0^p,\Delta t_p)\int{ \sigma_{i,j}^{S}(\lambda)\cdot I_{pulse}(\lambda)\cdot (\lambda/hc)d\lambda}
\end{equation}
Here, the rate coefficient has a temporally invariant spectral component given by the pulse photon flux (the pulse spectral intensity from equation~\ref{Eq:OG:SpecIntensity} divided by the energy per photon ($hc/\lambda$)) and the absorption/emission cross-section ($\sigma_{1,2}^{S}(\lambda)$ is the absorption spectrum of state $P_R$ or $P_{FR}$ in $cm^2$, while $\sigma_{3,4}^{S}(\lambda)$ is the stimulated emission spectrum).
The invariant spectral component is multiplied by the temporal intensity envelope of the pulse given in equation~\ref{Eq:OG:TempIntensity}. Combined, the product of the two functions in Equation~\ref{Eq:OG:TempIntensity} gives a time dependent rate coefficient for the optically coupled transitions.

The final term in equation~\ref{ER1} ($k_{LF5\rightarrow R1}$) is the gain term from $LF5$ to $R1$ that mediates the {reverse} switching from $P_{FR}$ to $P_{R}$ by way of the transient intermediate LUMI-F.
The final term in equation~\ref{ER5} ($k_{LR5\rightarrow FR1}$) is the loss term from LR5 to $FR1$ that mediates the {forward} switching from $P_{R}$ to $P_{FR}$ by way of the transient intermediate LUMI-R.
These terms are present in the corresponding equations for the dynamics of the $P_{FR}$ levels LF5 (eq.~\ref{EFR5}) and FR1 (eq.~\ref{EFR1}), acting as loss and gain terms, respectively. The $k_{LR5\rightarrow FR1}$ and $k_{LF5\rightarrow R1}$ rates are much smaller than the other rate constants (more than \emph{eight} orders of magnitude). This distinction arises because the large scale reorientation of the protein domains associated with the transformation from the transient intermediate products to the final product states occurs on a completely different time scale than the initial photo-isomerization (hundreds of microseconds compared to a few picoseconds).
When calculating the time dependent level populations the $k_{LR5\rightarrow FR1}$ and $k_{LF5\rightarrow R1}$ rates are effectively zero, and the final transient product populations at the end of the simulated time must be handled by a separate calculation to give the final product state populations. %\mbox{([\pr]\sub{fin},[\pfr]\sub{fin})=(R1\sub{fin}}, FR1\sub{fin}).
The inclusion of the latter rates here serve to link the ODEs that describe the $P_R$ levels (equations~\ref{ER1}-\ref{ER5}) to the ODEs that describe the $P_{FR}$ levels (equations~\ref{EFR1}-\ref{EFR5}).
As stated earlier, the transfer from the intermediate states (LR5 and LF5) are 100\% efficient, with the entire accumulated population of LR5 and LF5 at the end of the simulated time being added to FR1 and R1, respectively, to complete the simulated photoswitching reaction with all switches in one of the two ground states.
%not shown, but equivalent in form to equations~\ref{ER1}-\ref{ER5}).

Solving the set of rate equations above gives the dynamic populations of the indicated levels. The two sets of five dynamically coupled ODEs were solved using Matlab's ODE45 solver, based on the explicit Runge-Kutta (4,5) integrator from references~\cite{Dormand1980, Shampine1997}.
To avoid the differential equations becoming ``stiff'' the time domain of the calculation was broken into intervals, preventing rapid jumps in the magnitude of the time-varying optically coupled rate coefficients between steps of the algorithm.
The level populations are calculated over a sufficiently long time interval to allow the laser pulses to pass and the dynamic optically coupled rate coefficients to go to zero, taken as five pulse widths before the center of the first pulse and after the last pulse. After this time the equations are reduced to a simple exponential relaxation of the population excited during the optically driven dynamics back to the ground or transient levels. These relaxations can be analytically determined and the final product populations calculated directly once the results of the optically coupled transitions are computed.

With laser intensities of zero the dynamic rate equations for the \pr levels (equations~\ref{ER1}-\ref{ER5}) and the \pfr levels (equations~\ref{EFR1}-\ref{EFR5}) simplify to the following analytically solvable first order rate equations:
\begin{subequations}
\label{EqSteady}
\begin{align}
  \dfrac{d(R1(t))}{dt} ={}& k_{3,1}^R\cdot R3(t)
  \label{ESR1}\\
  \dfrac{d(R3(t))}{dt} ={}& -(k_{3,4}^R +k_{3,5}^R)\cdot R3(t)
  \label{ESR3}\\
  \dfrac{d(LR5(t))}{dt} ={}& k_{3,5}^R\cdot R3(t)
  \label{ESR5}\\
  \dfrac{d(FR1(t))}{dt} ={}& k_{3,1}^FR\cdot FR3(t)
  \label{ESFR1}\\
  \dfrac{d(FR3(t))}{dt} ={}& -(k_{3,4}^FR +k_{3,5}^FR)\cdot FR3(t)
  \label{ESFR3}\\
  \dfrac{d(LF5(t))}{dt} ={}& k_{3,5}^FR\cdot FR3(t)
  \label{ESFR5}
\end{align}
\end{subequations}

\noindent Here the transient levels 2 and 4 are removed, as any residual population of level 2 can be directly added to level 3, and level 4 can be bypassed without altering the final solution. The initial conditions of these reduced equations are set by the populations of the dynamic rate equation solutions at the end of the optically coupled time interval. For an intermediate level population at time $T_1$ of [$R1_1, R3_1, LR5_1,F1_1, F3_1, LF5_1$]  the post-exposure exponential dynamics and steady-state populations at long time are calculated to be:

\begin{subequations}
\label{Eqsteadyt}
\footnotesize
\centering
\begin{align}
  R3(t)={}&R3_1\cdot e^{-(k_{3,1}^R +k_{3,5}^R)t}{} &\Rightarrow&R3_{S.S.}=0
  \label{ETR3}\\
  R1(t)={}&R1_1+\dfrac{k_{3,1}^R}{k_{3,1}^R+k_{3,5}^R}R3_1\left(1-e^{-(k_{3,1}^R+k_{3,5}^R)t}\right) & \Rightarrow&R1_{S.S.}=R1_1+\dfrac{k_{3,1}^R}{k_{3,1}^R+k_{3,5}^R}R3_1
  \label{ETR1}\\
  LR5(t) ={}& R5_1+\dfrac{k_{3,5}^R}{k_{3,1}^R+k_{3,5}^R}R3_1\left(1- e^{-(k_{3,1}^R +k_{3,5}^R)t}\right){} & \Rightarrow&LR5_{S.S.}= R5_1+\dfrac{k_{3,5}^R}{k_{3,1}^R+k_{3,5}^R}R3_1
  \label{ETR5}\\
  FR3(t) ={}& F3_1\cdot e^{-(k_{3,1}^{FR} +k_{3,5}^{FR})t}{} & \Rightarrow&F3_{S.S.}=0
  \label{ETFR3}\\
  FR1(t)={}&F1_1+\dfrac{k_{3,1}^{FR}}{k_{3,1}^{F}+k_{3,5}^{FR}}F3_1\left(1-e^{-(k_{3,1}^{FR}+k_{3,5}^{FR})t}\right) & \Rightarrow&F1_{S.S.}=F1_1+\dfrac{k_{3,1}^{FR}}{k_{3,1}^{FR}+k_{3,5}^{FR}}F3_1
  \label{ETFR1}\\
  LF5(t) ={}& F5_1+\dfrac{k_{3,5}^{FR}}{k_{3,1}^{FR}+k_{3,5}^{FR}}F3_1\left(1- e^{-(k_{3,1}^{FR} +k_{3,5}^{FR)}t}\right) & \Rightarrow&LF5_{S.S.}= F5_1+\dfrac{k_{3,5}^{FR}}{k_{3,1}^{FR}+k_{3,5}^{FR}}F3_1
  \label{ETFR5}
\end{align}
\end{subequations}

\noindent The ``long time'' at which the system reaches these steady state intermediate populations is $\sim$nanoseconds after excitation, which is orders of magnitude longer than the $\sim$ picosecond excited state relaxation/isomerization but still orders of magnitude shorter than the final LUMI-R/LUMI-F relaxation occuring over $\sim$ microseconds.
Calculating the ground and transition state populations in this direct manner is much more rapid and reliable than running the ODE solver over the vastly different time-scales of the optically driven transitions and the subsequent post-exposure relaxation.
In the final step of the simulated photoswitching reaction, the accumulated transition state population is transferred to the switch's alternate ground state ($[P_{R}]_{fin}=R1_{S.S.}+LF5_{S.S.}$ and $[P_{FR}]_{fin}=FR_{S.S.}+LR5_{S.S.}$). This completes a single photoswitching reaction from a single dual-pulse excitation-depletion exposure iteration.
Section~\ref{Sec:OG:REMMulti} describes how this final product state population distribution can subsequently be used as a new initial population condition, allowing the simulated photo-reaction to be repeated, replicating the gradual transfer of larger populations over multiple exposures.
This is representative of the experiments performed in Section~\ref{Sec:OG:SDQExp},
where the sample is exposed to many Excitation-Depletion pulse pairs in a single measurement, specified by the measurement time and the repetition rate of the laser, to iteratively accumulate a larger final product population.

% %% INTRODUCE THE CHARACTERISTIC COEFFICIENTS

For characterizing the effect of the depletion pulse in the selective quenching of the forward and reverse photoswitching reactions, it is useful to monitor not just the final product populations, but also the fraction of the population taking part in the forward and reverse reactions.
To this end, we define the transformation of the initial state population distribution to the final product state populations in terms of a set of ``\emph{characteristic coefficients}'': the forward and reverse Yield Coefficients ($Y_{R,FR}$ \& $Y_{FR,R}$) and the forward and reverse Quenching Coefficients ($Q_R$ \& $Q_{FR}$).
\begin{subequations}\label{eq:Sim:CharCoeffs}
  \begin{align}
    P_{R,f}={}&\left(1-(1-Q_R ) Y_{R,FR} \right)P_{R,f} + \left((1-Q_{FR} ) Y_{FR,R} \right)P_{FR,i}\\
    P_{FR,f}={}&\left((1-Q_R ) Y_{R,FR} \right)P_{R,i} + \left(1-(1-Q_{FR} ) Y_{FR,R} \right)P_{FR,i}
    \end{align}
\end{subequations}
\noindent Here, the per exposure yield in the forward direction, ${Y_{R,FR}}$, is defined as the fraction of molecules transferred from \pr to \pfr by the excitation pulse alone and the forward quenching coefficient, ${Q_R}$, is the relative change in forward yield brought on by the interaction with the depletion pulse; the corresponding reverse coefficients ${Y_{FR,R}}$ and ${Q_{FR}}$ are defined for the reverse reaction in the same way.
Importantly, these \emph{characteristic coefficients} are independent of the population distribution of the sample, being exclusively related to the variable experimental control parameters used to define and describe the excitation and depletion laser pulse pair.
In this way the \emph{characteristic coefficients} serve as a link between the control parameters and the optogenetic switch product output.
It is straightforward to see that the ratios of the steady-state isomerization product populations to the initial state populations are equal to the product of the yield and quench coefficients for the forward and reverse reactions, respecively:
\begin{subequations}\label{eq:Sim:LumiCCs}
  \begin{align}
    LR5_{S.S.}/R1_0={}&\left(1-(1-Q_R ) Y_{R,FR} \right)\\
    LF5_{S.S.}/FR1_0={}&\left(1-(1-Q_{FR} ) Y_{FR,R} \right)
    \end{align}
\end{subequations}
This parallel will serve as a useful means to extract information about the transient intermediate level populations without requiring ultrafast absorption measurements during the experiments presented in Section~\ref{Sec:OG:SDQExp}.
The Net Gain of \pfr for a single photoswitching event is the difference between the forward and reverse reaction products:
\begin{equation}\label{eq:OG:netgain}
  \Delta P_{FR} = (1-Q_{R})Y_{R,FR}\cdot P_{R}-(1-Q_{FR})Y_{FR,R}\cdot P_{FR}
\end{equation}

%%%% Time to Plot Some Graphs!
To illustrate the output of the simulation, Figure~\ref{UFDynamics} shows the un-depleted dynamic level populations of a system exposed to only the short-pulsed excitation.
The system in Figure~\ref{UFDynamics} is composed of an initial equal mixture of states, $[P_{R}]_{init.}=[P_{FR}]_{init.}=0.5$  (this initial condition is arbitrary and chosen for these figures to show the dynamics of both states on the same scale).
These dynamic level populations are plotted in the short, optically coupled time interval as well as the long, post-exposure relaxation time domain.
At t=0ps the $P_R$ and $P_{FR}$ populations of the system are exposed to the excitation pulse with 100 fs duration and 30 nm spectral bandwidth centered at 625 nm, the average power is 0.50 mW corresponding to a peak intensity of 18.69 \nicefrac{GW}{cm\up2}.
The temporal envelope of the excitation pulse is shown in the figure as the shaded Gaussian profile.
\begin{figure}
  \centering
  \includegraphics[width=.9\linewidth]{ch-OG/Figs/REM/Figure_UFDynamics}
  \caption[Modeled Ultrafast Un-Depleted Dynamics]{Un-depleted dynamic populations of the five levels of each switch state ((a) $P_{R}$ and (b) $P_{FR}$) with the excitation pulse envelope (yellow area).
  In both (a) and (b) the laser excitation pulse has zero intensity by 0.5 ps (five pulse widths) and the remaining dynamics are described by exponential relaxation from the lower level of the excited state (level~3, green trace) to the transient product state (level~5, red trace) or back to the initial ground state (level~1, blue trace, by way of level~4, teal trace). The distinctions between figures (a) and (b) highlight the much faster dynamics of $P_{FR}$ compared to $P_{R}$. Excitation laser parameters associated with the figure are listed in the text and Table~\ref{Table:OG:LaserParam}. For this excitation pulse, the single exposure Net Gain of $\Delta P_{FR}=+0.046$ or 9.1\% of the initial \pfr population.}
  \label{UFDynamics}
\end{figure}
It must be noted here that, for illustration purposes within this figure, the power of this excitation pulse is exceptionally high. To make the features of the level dynamics more distinguishable and to highlight the alteration of those dynamics achieved by the stimulated depletion quenching, the powers of the excitation and depletion pulses in Figures~\ref{UFDynamics} and \ref{UFDeplete} are at the upper range of powers examined in this study.
In Figure~\ref{UFDynamics} the total excited state populations ($P_{R}$*=R2+R3, $P_{FR}$*=FR2+FR3) are plotted as the thicker, darker green trace to illustrate how the excited state mirrors the ground state bleach initially, as well as to illustrate how the excited population moves from the initial upper excited level 2 (red trace) to the vibrationally relaxed level 3 (thin green trace).

%\footnote{listing \emph{Peak} Intensity ([0.94*Avg Power/RepRate/$\uptau_{width}$]/area)=18.69 \nicefrac{GW}{cm\up2}. (A) Do I need to re-state this relation or is it enough that it's in Eq.~\ref{Eq:OG:TempIntensity}? (B) Could also list \emph{Average} Intensity (Avg Power/area), but Peak Intensity is the valid param, right? } .


Looking at the optically coupled time domain in Figure~\ref{UFDynamics} it is clear that, as measured in studies of the actual chromophore, the reverse isomerization reaction is much more rapid than the  forward isomerization. The $P_{FR}$ excited state (FR3) has already peaked by $\sim0.1$ ps after the excitation begins and by 1 ps has nearly completely converted to the LUMI-F transient product (LF5) or back to the ground state (FR1).
In contrast, around 1 ps the $P_{R}$ excited state R3 is still growing from population stored in R2, and very little population has switched to the transient state LR5. The switch in the $P_{R}$* state does not fully isomerize to LR5 or return to the ground state R1 for over 100 ps.
The steady state level populations, as well as the final product state populations and forward and reverse Yield coefficients are shown on the figure beside each graph.
For the excitation only exposure in Figure~\ref{UFDynamics} the Quenching coefficients are zero and the Net Gain is $\Delta P_{FR} = 0.0456$ or 9.126\%.


The ultrafast dynamics of the $P_{FR}$ photo-isomerization forces us to keep the depletion pulse short and very close to the excitation pulse to quench the reaction before it forms the transient LUMI-F product. Rather than being a preventative factor, these distinct dynamics allow us to entirely deplete the $P_{FR}$* excited state before the excited $P_{R}$* population has fully relaxed from the initial excitation point. This gives a window to halt the reverse reaction without fully stopping the forward reaction.
The shorter interaction time of the depletion pulse limits the amount of stimulated depletion possible per exposure, restricting the maximum Quenching coefficient; but by cycling many exposures this advantage can drive the equilibrium in favor of the $P_{FR}$ photo-product.



\begin{table}
  \centering
  \begin{tabular}{@{}l c c c c c}
    \toprule
    \thead{Laser Pulse}&\thead{$\mathbf{\langle P\rangle}$(mW)}&\thead{$\mathbf{\lambda_0}$ (nm)}&\thead{$\mathbf{\Delta \lambda}$ (nm)}&\thead{$\mathbf{\Delta t_{width}}$ (ps)}&\thead{$\mathbf{t_{Ex,Dep}}$ (ps)}\\
    \midrule
    Excitation&0.50&625&30&0.10&n/a \\
    Deplet. 775nm&10.0&775&10&0.140&0.080 \\
    Deplet. 835nm&10.0&835&10&0.140&0.080 \\
    \bottomrule
  \end{tabular}
  \caption[Model Laser Parameters]{Collective laser parameter settings for simulating laser excitation and depletion pulses in Figures~\ref{UFDynamics}, \ref{UFDeplete}, and \ref{Fig:MultiExp}.
  Average power ($\langle P\rangle$), central wavelength ($\lambda_0$) and spectral width ($\Delta \lambda$), temporal duration ($\Delta t_{width}$) and excitation-depletion delay ($t_{Ex,Dep}$) used in the calculation of pulse intensities by Eq.~\ref{Eq:OG:SpecIntensity} and Eq.~\ref{Eq:OG:TempIntensity}. These laser pulse intensities are exceptionally high, and used here only for illustration purposes. It is shown later that similar results can be achieved with lower pulse intensities. }
\label{Table:OG:LaserParam}
\end{table}



Figure~\ref{UFDeplete} shows the altered dynamics after excited state quenching at two different depletion wavelengths.
To simplify the graphs, the figure shows the summed populations of the levels to represent the populations of the ground states ($R1+R4=P_{R}$, $FR1+FR4=P_{FR}$), excited states ($R2+R3=P_{R}$*, $FR2+FR3=P_{FR}$*), and intermediate product states (LR5=LR, LF5=LF).\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{ch-OG/Figs/REM/Fig_UFDeplete}
  \caption[Modeled Ultrafast Depletion]{Comparing depleted dynamics of the $P_{R}$ (a) and $P_{FR}$ (b) states at two depletion wavelengths. The ground-state bleach ($-\Delta P_{R},-\Delta P_{FR}$), excited state ($P_{R}$*$,P_{FR}$*), and transient product (LR,LF) populations  of each state are plotted along with the excitation and depletion pulse envelopes (yellow and pink, respectively).
  The forward and reverse Yield and Quenching coefficients, and the final net Gain of \pfr are listed below the key for each exposure condition.
  For the depletion at 835 nm with $Q_{FR}\sim(2\!\times\!Q_{R})$, effectively halting the reverse reaction while allowing the forward reaction to proceed. This produces a lower Gain per exposure, but will shift the photoequilibrium. The depletion at 775 nm quenches forward and reverse reactions equally.
  Laser parameter settings are listed in the text and Table~\ref{Table:OG:LaserParam}.} \label{UFDeplete}
\end{figure}
%Stimulated depletion of the excited state reduces the transient products and recovers the ground state population.
The excitation pulse and initial $P_R$ and $P_{FR}$ populations are the same as used in Figure~\ref{UFDynamics}, and the un-depleted level dynamics are plotted in the figure as solid lines. The dynamic level populations from two separate excitation-depletion exposures are shown, one with a central depletion wavelength of 775 nm (dashed traces) and the other centered at 835 nm (dotted traces), both with 10 nm bandwidth. The depletion pulses both have temporal full width at half max of 0.140 ps duration and arrive at a delay of 0.080 ps after the excitation pulse. The average power of both depletion beams is 10.0 mW corresponding to a peak intensity of 150 \nicefrac{GW}{cm\up2}.%\footnote{Peak Intensity 150 \nicefrac{GW}{cm\up2} or Avg Intensity 32 \nicefrac{W}{cm\up2}?}.
As stated before, this intensity is exceptionally high to emphasize the effects of the stimulated depletion quenching in the figure.
It is shown later in Section~\ref{Sec:OG:REMSurvey} that similar final populations can be obtained with appropriate pulses of lower power.


The forward and reverse Yield and Quench coefficients and the \pfr Net Gain are shown on Figure~\ref{UFDeplete} by the key for each exposure condition. These values, as well as the final populations of the \pr and \pfr states, and the steady-state populations of the LUMI-R and LUMI-F transient states are collected in Table~\ref{Tab:ModResults}.
The final \pr and \pfr populations include the transfer of the accumulated population of the transient states to their final product ground states. The laser parameters associated with these results are collected in Table~\ref{Table:OG:LaserParam} for reference.


\begin{table}
  \centering
  \begin{tabular}{@{}l c c c c c c c}
    \toprule
    \thead{Exposure\\ Condition\\{}}&\thead{Final \\ $\mathbf{P_{R}}$\\{}}&\thead{Final \\ $\mathbf{P_{FR}}$\\{}}&\thead{Net Gain\\ $\mathbf{\Delta P_{FR}}$\\{}} & \thead{LUMI-R \\ (${LR5_{S.S.}}$)\\{}} & \thead{LUMI-F \\ (${LF5_{S.S.}}$)\\{}} &\thead{Forward \\ Quench \\ $\mathbf{Q_R}$}&\thead{Reverse \\ Quench \\ $\mathbf{Q_{FR}}$}\\
    \midrule
    Un-Depleted&0.454&0.546&9.1\%&.0742&.0285& -- & -- \\
    Deplet.775nm&0.481&0.519&3.7\%&.0306&.019&58.7\%&58.2\%\\
    Deplet.835nm&0.461&0.539&7.7\%&.0438&.0052&41.0\%&81.9\%\\
    \bottomrule
  \end{tabular}
  \caption[Model Results: Yield and Depletion]{Collective results from exposure of an initial 50/50 mixed state to a single excitation-depletion pulse pair.
  The final populations are listed in the first two columns, followed by the Net Gain of the \pfr state. The intermediate steady-state populations of the transient isomerization products are next; followed by the Quenching coefficients, which give the percent change in the transient population with and without depletion.The forward/reverse Yield coefficients from the excitation pulse for all conditions are $Y_{R,FR}=14.83\%$ and $Y_{FR,R}=5.703\%$, respectively}
    \label{Tab:ModResults}
\end{table}

Quenching of the photo-isomerization is achieved at both depletion wavelengths for both states, as demonstrated by the drop in transient product states (levels LR5 and LF5, red in both graphs in Figure~\ref{UFDeplete}) and recovery of the initial ground states (levels R1 and FR1, blue in both graphs).
Looking at the values in Table~\ref{Tab:ModResults}, we see that SDQ \emph{lowers} the Net Gain ($\Delta P_{FR}$) per exposure for both depletion pulses, which would seem to run counter to our objective.
However, we will see that the $\Delta P_{FR}$ per exposure is less consequential than generating a significant difference between the Forward and Reverse Quenching Coefficients, $Q_{FR}\gg Q_{R}$.
The shorter wavelength depletion pulse ($\lambda_{0,D}= 780$ nm) quenches both $P_{R}$* and $P_{FR}$* excited states equally, $Q_{FR}\simeq Q_{R}$. This only slows the overall reaction, giving no selective control between the forward and reverse reaction directions.
%, giving a low \pfr Net Gain of 3.75\%,
The longer wavelength depletion pulse ($\lambda_{0,D}= 835$ nm) nearly completely depletes the $ P_{FR}$* excited state before much transient product can form, while the $ P_{R}$* excited state retains some population that continues the forward reaction.
This results in a lower Net Gain per exposure than the un-depleted excitation, $\Delta P_{FR}=7.72\%<9.13\%$, but nearly no loss of $P_{FR}$ to the reverse reaction.
It will be shown next in Section~\ref{Sec:OG:REMMulti} that this shift in the balance of the forward and reverse reactions enhances the maximum $P_{FR}$ population achieved at photoequilibrium over multiple exposures.

%$P_{FR}$*
These single exposure simulations show that with moderate laser parameters attainable experimentally it is reasonable to expect depletion of the excited state of the PCB chromophore in Cph8 before photo-isomerization occurs, thereby quenching the (\pfr$\rightarrow$\pr) reverse photoswitching reaction. The simulations further show that the extremely rapid dynamics of the $P_{FR}\rightarrow P_R$ photo-isomerization, rather than being a hindrance to control, allows selective depletion of the $P_{FR}$* excited state without complete depletion of the $P_{R}$* excited state, enabling favorable quenching of the reverse $P_{FR}\rightarrow P_R$ photoswitching and relative enhancement of the forward $P_{R}\rightarrow P_{FR}$ reaction.
Next, simulations of the system exposed to multiple repeating laser exposures will show that the SDQ enhancement shifts the photoequilibrium, greatly increasing the dynamic range of the switch.

%% End Single Pulse Simulation, Begin Multipulse Simulation
%#####################################################################################
%#####################################################################################
%#####################################################################################
%#####################################################################################
%#####################################################################################
%#####################################################################################
%#####################################################################################
%\pagebreak
%\subsection*{Iterative Mapping}
%
%For a generic system converting between two states with a conserved population and a fractional yield per iteration from state $m$ to state $n$ of $X_{mn}$, the population can be described:
%\begin{equation}\label{}
%\begin{split}
%   &C_0 [X_{10} \leftrightarrows X_{01}] C_1 \\
%    C_{0,f} =& X_{10}C_{1,i} + (1-X_{01})C_{0,i} \\
%    C_{1,f} =& X_{01}C_{0,i} + (1-X_{10})C_{1,i}.
%\end{split}
%\end{equation}
%\noindent The yield terms $X_{mn}$ are independent of the state of the system or population distribution, in our experiments these are defined by the laser control parameters. The expression above can be expressed as the matrix equation:
%\doublespacing
%\begin{equation}\label{}
%  \begin{split}
%     \mathbf{C_f} &= \underline{\underline{\mathbf{M}}}\cdot \mathbf{C_i} \\
%     \binom{C_{0,f}}{C_{1,f}}  &=  \begin{bmatrix}
%                                     (1-X_{10}) & X_{01} \\
%                                     X_{10} & (1-X_{01}) \\
%                                   \end{bmatrix}
%     \cdot \binom{C_{0,i}}{C_{1,i}}
%  \end{split}
%\end{equation}
%\noindent This 2x2 matrix has algebraically solvable eigensolutions. For T defined as the Trace of the matrix and D defined as the matrix determinant, the eigenvalues are given by
%
%\begin{equation}\label{}
%  \begin{split}
%     \lambda_{\pm} &= T/2 \pm \sqrt{(T/2)^2 - D} \\
%      \overline{v_{\pm}} &= \binom{b}{\lambda_{\pm} - a}
%  \end{split}
%\end{equation}
%
%which gives:
%
%\begin{equation}\label{}
%  \begin{split}
%     \lambda_1 =& 1 &v_1 = \dfrac{1}{X_{10}+X_{01}}*\binom{X_{01}}{X_{10}}\\
%     \lambda_2 =& 1-(X_{10}+X_{01}) &v_2 = \dfrac{1/2}{1/2}
%  \end{split}
%\end{equation}
%
%\doublespacing
%\pagebreak
%
%%#####################################################################################
%#####################################################################################
%#####################################################################################
%#####################################################################################
%#####################################################################################
%#####################################################################################
%#####################################################################################


%Developing the Optical Transformation Matrix to Simulate Multiple Exposures
\subsection{Simulating Multiple Exposures with the Optical Transformation Matrix}\label{Sec:OG:REMMulti}
%After simulating the dynamics of the system with a single excitation-depletion pulse sequence the final populations of the chromophore in states $[P_{R}]_{fin.}$ and $[P_{FR}]_{fin.}$ are then set as the new initial conditions of the rate \nohyphens{equations~\ref{ER1}-\ref{EFR5}} and the simulation could be repeated, incrementally transferring population between the $P_R$ and $P_{FR}$ states over many simulated exposures.
%This method of repeatedly solving the set of differential Rate Equations hundreds of times is not only slow, it is also prone to calculation errors due to round-off approximations and inaccuracies of the ODE solver. A better method is to recognize that this transfer of the initial state populations to the final state populations can be represented as a linear transformation of a vector of state populations by an \emph{Optical Transformation Matrix} (OTM) \textbf{T}:

The simulations of the last section determine the final population of a system ($P_{R,f}, P_{FR,f}$) after exposing an initial population ($P_{R,i}, P_{FR,i}$) exposed to a single Excitation-Depletion pulse sequence, defined by a set of laser control parameters, by solving a set of differential rate \nohyphens{equations~\ref{ER1}-\ref{EFR5}}.
To determine the results of multiple exposures, rather than repeatedly solving the ODEs with new initial conditions at each iteration
(which is not only slow, but also prone to calculation errors due to round-off approximations and inaccuracies of the ODE solver)
it is more convenient to to represent the transfer of the population of the system from an initial state to a final state as a linear transformation of a vector of state populations by an \emph{Optical Transformation Matrix} (OTM) \textbf{T}:

%\singlespacing
\begin{equation}\label{Eq_OTM}
 {\bf P_{f}}=\begin{bmatrix}
          P_{R,f} \\
          P_{FR,f} \\
        \end{bmatrix} =\begin{bmatrix}
                        T_{1,1} & T_{1,2} \\
                        T_{2,1} & T_{2,2}
                      \end{bmatrix} \cdot \begin{bmatrix}
          P_{R,i} \\
          P_{FR,i} \\
        \end{bmatrix}  = \textbf{T} \cdot {\bf P_{i}} \ .
\end{equation}

%\doublespacing

\noindent
The introduction of the OTM and its identification in the laboratory (reported in Section~\ref{Sec:OG:Results}) is a key feature of the experiments in this work.
The elements of the OTM are independent of the initial population distribution, as they are defined solely by the laser control parameters.
Because of the complexity of the interactions, it is prohibitively difficult to directly calculate the matrix elements from the optical response functions of the molecule and laser parameters. To compute the values of the matrix elements we simulate a single iteration of the transformation using the rate equation ODEs, as described in Section~\ref{Sec:OG:REMSingle}, for two particular initial conditions and then solve for the matrix elements from the relationship between the initial and final populations. This reduces the number of times we must solve the rate equation system of ODEs from hundreds to just two.
Similarly, in the experiments of Section~\ref{Sec:OG:SDQExp} the OTM formalism allows us to extrapolate to the final equilibrium population distribution after measuring a smaller number of laser exposures. In this way we can measure the SDQ enhancement of a larger laser control space, without having to wait for each permutation of the control parameters to reach photoequilibrium.
In the simulations, we are able to solve the rate equations using the two initial conditions $\bigl[\begin{smallmatrix} 1 \\ 0 \\ \end{smallmatrix}\bigr]$ and $\bigl[ \begin{smallmatrix} 0 \\ 1 \\ \end{smallmatrix}\bigr]$, which provides the matrix elements directly:

%\singlespacing
\begin{equation}\label{Eq_OTMelements}
  \mathbf{T}\cdot \begin{bmatrix}
                             1 \\
                             0 \\
                           \end{bmatrix} = \begin{bmatrix}
                             T_{1,1} \\
                             T_{2,1} \\
                           \end{bmatrix} \textrm{, and }\mathbf{T}\cdot \begin{bmatrix}
                             0 \\
                             1 \\
                           \end{bmatrix} = \begin{bmatrix}
                             T_{1,2} \\
                             T_{2,2} \\
                           \end{bmatrix}
\end{equation}

%\doublespacing

\noindent highlighting the practical definition of the OTM elements: the off-diagonal elements $T_{1,2}$ and $T_{2,1}$ are the fractional gain per exposure between the two states.
%\pr to \pfr state (Forward Yield: $Y_{R,FR}$) and from the \pfr to the \pr state (Reverse Yield: $Y_{FR,R}$), respectively.
We could also refer to the definition of the \emph{characteristic coefficients} in Equation~\ref{eq:Sim:CharCoeffs} and write the OTM relation as:

%\singlespacing
\begin{equation}\label{eq:OG:OTMccs}
\small
 \begin{bmatrix}
          P_{R,f} \\
          P_{FR,f} \\
        \end{bmatrix} =\begin{bmatrix}
                        (1-(1-Q_{R})Y_{R,FR}) & (1-Q_{FR})Y_{FR,R} \\
                        (1-Q_{R})Y_{R,FR} & (1-(1-Q_{FR})Y_{FR,R})
                      \end{bmatrix} \begin{bmatrix}
          P_{R,i} \\
          P_{FR,i} \\
        \end{bmatrix}
\end{equation}

%\doublespacing
\noindent To calculate the transfer of population from an arbitrary state distribution over a series of exposures the initial population vector is simply multiplied by, $\mathbf{T}^N$, the OTM raised to the number of exposures.
This iterative transfer of population over many laser exposures is possible because the population distribution of the system does not change between iterations when the period between laser pulses is less than the dark-relaxation time of the switch (minutes to hours for Cph8 \cite{Psakis2011}).
This gradual population transfer is plotted in Figure~\ref{Fig:MultiExp}. The system begins in the pure $P_{R}$ state $\bigl[\begin{smallmatrix} 1 \\ 0 \\ \end{smallmatrix}\bigr]$ and is exposed to three different exposure conditions: un-depleted single-pulse excitation, and two sets of sequential excitation-depletion exposures with a depletion pulse centered at 775 nm and 830 nm.
The laser parameters for Figure~\ref{Fig:MultiExp}, collected in Table~\ref{Table:OG:LaserParam}, are the same as those used to plot Figures~\ref{UFDeplete} and \ref{UFDynamics}.
%The excitation pulse has average power 0.50 mW, spectral width of 30 nm centered at 625 nm, and temporal duration 100 fs. The depletion pulses both have average power 10 mW, spectral width of 10 nm, and temporal duration 140 fs. The excitation-depletion delay is 80 fs for both depletion pulses.
\begin{figure}
  \centering
  \includegraphics[width=.9\linewidth]{ch-OG/Figs/REM/Fig_MultiExp}
  \caption[Modelled Multi-Exposure Accumulation of Photo-product]{Multi-exposure photo-isomerization yield with an un-depleted linear exposure, and an excitation-depletion pulse sequence exposure at two separate depletion wavelengths. In the first few exposures the faster reaction rate of the un-depleted exposure enables greater $P_{FR}$ generation, but after several exposures the quenching enhancement allows the sample exposed to the depletion at 830 nm to overcome the linear equilibrium limit and eventually reach a new equilibrium at $\sim$90.2\%. Laser parameters are listed in the text.}\label{Fig:MultiExp}
\end{figure}
The photoequilibrium threshold (i.e., the maximum \pfr or minimum \pr population) under each exposure condition is annotated on the figure. Also noted are the forward and reverse Yield associated with the excitation pulse and the forward and reverse Quenching coefficients for each depletion pulse wavelength.
%the stimulated depletion quenching coefficient $Q_{i,f}$, the percent change in per pulse yield from state \emph{i} to state \emph{f} due to SDQ and the un-depleted yield: $Q_{i,f}= \left(\nicefrac{\left(Y_{i,f}^{(Ex)}-Y_{i,f}^{(ExDp)}\right)}{Y_{i,f}^{(Ex)}}\right)$.}Under un-Depleted red-light exposure the sample stabilizes at a photo-equilibrium threshold: 72.22\% $P_{FR}$ 27.78\% $P_{R}$.
When the sample is exposed to the excitation-depletion pulse pair, with the depletion pulse centered at 775 nm, the depletion cross-section is similar for both states of the chromophore, and the quenching parameters of the forward and reverse reaction are nearly identical ($Q_{R,FR} = 58.7\%, Q_{FR,R} = 58.2\%$). As a result, the depletion produces a small increase in the final equilibrium (74.63\% $P_{FR}$ 25.37\% $P_{R}$); but mainly serves to slow the reaction, increasing the number of exposures to reach 90\% of the equilibrium threshold ($N_{DEC}$) from 11 to 28 exposures.
When the central wavelength of the depletion pulse is 835 nm the photoswitching reaction continues rising past the linear threshold to a new enhanced equilibrium.
Initially, the slower reaction rate of the selectively quenched photoswitching produces less $P_{FR}$ than the standard linear excitation; however, after $\sim$20 exposures the quenched photoswitching reaction surpasses the cross-talk limited linear excitation threshold, achieving the final product population of 90.25\% $P_{FR}$ and 9.75\% $P_{R}$.
% with a set of depletion pulse parameters of 10 nm bandwidth at a central wavelength of 840 nm, a temporal pulse width of 0.14 ps, and an excitation-depletion delay of 0.06 ps.
This selective depletion significantly enhances the final yield of the desired $P_{FR}$ product and decreases the undesired $P_{R}$ product by a factor of 4 compared to the linear exposure limit.

Another feature of the iterative mapping formulation of the photoswitching process is that it is possible to solve for the associated eigenvectors and eigenvalues of the OTM:

%\singlespacing
\begin{equation}\label{Eq_Eigensols}
  \textbf{T}\cdot \textbf{v}_n = \lambda_n \textbf{v}_n
\end{equation}

%\doublespacing
\noindent which hold valuable information.
%For a simple 2x2 matrix we can directly calculate the eigensolutions. For a matrix
%
We know from the physics of the photoswitching reaction that one of the eigensolutions will have an eigenvalue of 1 and be associated with the equilibrium state population, because once equilibrium is reached subsequent exposures no longer alter the population, so $\textbf{T}^N\cdot \textbf{v}_{eq}=1\cdot \textbf{v}_{eq}$. The set of eigenvectors of a matrix are linearly independent and span the associated space, meaning that any initial population vector can be expressed in this eigenbasis:

%%\singlespacing
%\begin{equation}\label{Eq_Eigenbasis}
%  \textbf{P}=\begin{bmatrix} P_{R}\\ P_{FR}\\ \end{bmatrix}=P_{R}\begin{bmatrix} 1\\ 0\\ \end{bmatrix}+P_{FR}\begin{bmatrix} 0\\ 1\\ \end{bmatrix}=c_{eq}\begin{bmatrix} R_{eq}\\ F_{eq}\\ \end{bmatrix}+c_{tr}\begin{bmatrix} R_{tr}\\ F_{tr}\\ \end{bmatrix}
%\end{equation}
%\singlespacing
\begin{equation}\label{Eq_Eigenbasis}
  \textbf{P}=\begin{bmatrix} P_{R}\\ P_{FR}\\ \end{bmatrix}=c_{eq}\begin{bmatrix} R_{eq}\\ F_{eq}\\ \end{bmatrix}+c_{tr}\begin{bmatrix} R_{tr}\\ F_{tr}\\ \end{bmatrix}
\end{equation}

%\doublespacing

\noindent and application of \textbf{T} to the population vector becomes simply:

%\singlespacing
\begin{equation}\label{Eq_Eigenbasis}
  \textbf{T}\cdot \textbf{P}=1\cdot c_{eq}\begin{bmatrix} R_{eq}\\ F_{eq}\\ \end{bmatrix}+ \lambda_{tr}\cdot c_{tr}\begin{bmatrix} R_{tr}\\ F_{tr}\\ \end{bmatrix}
\end{equation}
%\doublespacing

\noindent In this form it is clear that the second eigensolution is associated with the population that is transferred between states to take the initial population vector closer to the equilibrium eigenvector with each iteration of the transform.
The second eigenvalue $\lambda_{tr}$ is related to the number of exposures it takes to reach the equilibrium state.
From this eigenvalue we define the \emph{Decimation Count}, $N_{Dec}$, as  the number of exposures necessary to reduce the transitional population to less than 10\% of it’s initial value:

%\singlespacing
\begin{equation}\label{Eq_NDec}
  N_{Dec}=\dfrac{-1}{log_{10}(\lambda_{tr})}
\end{equation}
%\doublespacing

\noindent The decimation count is a useful metric of the effectiveness of a set of laser exposure parameters: a pulse pair that achieves a final equilibrium threshold of 100\% \pfr and 0 \% \pr but requires infinitely many pulses to reach this equilibrium is not practically useful.

Knowledge of the eigensolutions of the OTM provide a direct, simple means to calculate the photoequilibrium threshold and efficacy of a set of laser control parameters without having to \emph{calculate} or \emph{measure} the photoswitching product populations over many iterations until the system actually reaches the photoequilibrium.


\subsection{Parameter Space Survey Results}\label{Sec:OG:REMSurvey}

With the methods of calculating the photoswitching reaction product populations and final photoequilibrium threshold established in the previous sections, we survey the reduced space of laser control parameters that can be experimentally varied without complex pulse shaping to determine the dependence of the SDQ enhancement of the photoswitching reaction on these parameters independently and in concert.
Except where otherwise noted, the following surveys are conducted around a fixed starting point in the parameter space specified in Table~\ref{Tab:SurveyStart}.
The excitation and depletion pulse pair described in the table produces the highest SDQ enhancement accessible by varying the chosen control parameters, reaching an enhanced equilibrium population of $>90\%$ \pfr and $<10\%$ \pr with powers, spectra, and pulse durations accessible with the laser sources in our experimental facilities.
Increasing the pulse peak intensities can enable higher equilibrium dynamic range, however this is achieved at the expense of slower reactions taking much longer to reach equilibrium, as shown later in Figure~\ref{DepPowScan}. Above an excitation power of 1 mW or a depletion power of 10 mW increasing the pulse powers gives diminishing returns and enters an intensity range where the rate equation model used here will become increasingly inaccurate. While this location in the control space produces the best SDQ enhancement from a survey within this restricted parameter basis, it is emphasized that reaching full performance optimality will require more sophisticated quantum dynamics modelling and coherent pulse shaping guided by optimal feedback control algorithms in the laboratory to address and exploit the complex coherent dynamics of the system.
The present results should be viewed as illustrative of the effectiveness of the SDQ mechanism for enhancing the dynamic range of the switch.


\begin{table}
  \centering
  \begin{tabular}{@{}l c c c c c}
    \toprule
    \thead{Laser Pulse}&\thead{$\mathbf{\langle P\rangle}$(mW)}&\thead{$\mathbf{\lambda_0}$ (nm)}&\thead{$\mathbf{\Delta \lambda}$ (nm)}&\thead{$\mathbf{\Delta t_{width}}$ (ps)}&\thead{$\mathbf{t_{Ex,Dep}}$ (ps)}\\
    \midrule
    Excitation&0.20&625&30&0.100& -- \\
    Depletion&6.5&833&10&0.140&0.080 \\
    \bottomrule
  \end{tabular}
  \caption[SDQ  Laser Parameters]{Best laser parameters for SDQ enhancement of Cph8 dynamic range based on a few-parameter survey of the control space.
  For this parameter set, SDQ enhanced the photoequilibrium to 90.25\% \pfr / 9.75\% \pr. Increasing the pulse powers can always increase the dynamic ranges, though at the expense of slower reactions and higher decimation count, $N_{DEC}$. Fully optimized control of the switches to their maximum dynamic range will require more elaborate quantum models and proper shaping of the laser pulse pairs in SDQ.}
\label{Tab:SurveyStart}
\end{table}

We first scan over a range of excitation pulse parameters with no Depletion pulse to confirm that the model behaves as expected in the single pulse, linear regime.
In Figure~\ref{ExWLScan} the central wavelength of the excitation pulse is varied to confirm that the photo-reaction fully resets the switch to the \pr state under far-red illumination and reaches a photoequilibrium between \pr and \pfr under red illumination.
For the measurements in the figure the excitation power was 0.20 mW, the pulse duration was 100 fs, and the spectral width was 30 nm while the central wavelength of the excitation spectrum was varied from 550 nm to 800 nm.
For wavelengths longer than 725 nm the equilibrium population of the \pr state is $[P_{R}]_{EQ}>99\%$, and for wavelengths in the red (600 nm $< \lambda <$ 670 nm) the final photoequilibrium ranges from 60-75$\%$ \pfr.
The photostatic equilibrium at shorter wavelengths is higher than measured for the Cph1 molecule (65-67$\%$). Looking at the decimation count $N_{DEC}$ of the system (inset in the figure) we see that for $\lambda <$610 nm the exposures necessary to reach equilibrium begins rising rapidly, due to the diminished absorption cross-section at these shorter wavelengths. If we cap the number of exposures at N=20, the value where the decimation count starts to rise divergently, we see that the photoequilibrium rises to $\sim$65$\%$ \pfr in the red spectral region before falling again as the molecule stops absorbing the shorter wavelength light.
Because the absorption spectra of the chromophores is so much broader than the width of the excitation or depletion spectra varying the spectral width of the excitation pulse has little effect on the photoswitching behavior. The molecule still fully resets to \pr under far-red illumination and reaches the same photoequilibrium under red illumination, increasing the spectral width only smears out the transition between these two regions of the molecular response, as shown in Figure~\ref{ExDWLScan}.
Varying the pulse temporal duration similarly has essentially no effect on the single-pulse photoswitching reaction.
With the excitation pulse power fixed at 0.20 mW and the spectrum centered at 625 nm with a bandwidth of 30 nm, stretching the pulse from 20 fs to 2 ps changes the equilibrium population by $\sim2\%$.
Having confirmed that the model returns the expected results in the linear, single-pulse exposure conditions we can begin to test the dependence on the depletion pulse parameters.

\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{ch-OG/Figs/REM/ExWLscan}
  \caption[Excitation wavelength dependence of photoswitching]{Excitation wavelength dependence of photoswitching under the condition of single pulse, linear excitation. Far-red light ($\lambda > 725 nm $) resets the system to the pure \pr state, while red light (600 nm $< \lambda <$ 670 nm) reaches a photoequilibrium between 60-75$\%$ \nicefrac{\pfr}{\pr}. At wavelengths with low absorption cross-section the final equilibrium population (dashed lines) becomes numerically unreliable as the excitation pulse interacts less with the molecule and the decimation count $N_{DEC}$ (inset) rises rapidly. For this reason we cap the number of exposures at 20 and look as the behavior of the system (solid lines), which reach the expected photoequilibrium of 65\% \pfr.
  }
  \label{ExWLScan}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.7\linewidth]{ch-OG/Figs/REM/scanExDWL}
  \caption[Spectral width dependence of photoswitching]{Varying the spectral width of the excitation pulse has little effect on the photoswitching reaction. The switch still resets under far-red illumination and comes to the same photoequilibrium under red illumination, but the transition between these two regions is less distinct as the excitation spectrum is broadened.}
  \label{ExDWLScan}
\end{figure}

%Next we scan over the excitation power to confirm that the system reaches the same equilibrium value regardless of excitation power (!!EXCEPT IT DOESN'T!!)
%\begin{figure}
%  \centering
%  \includegraphics[width=\linewidth]{ch-OG/Figs/REM/ExPscan}
%  \caption[Excitation power dependence of photoswitching]{Excitation power dependence of photoswitching}\label{ExWLScan}
%\end{figure}

The depletion pulse central wavelength was scanned over a series of values to find the optimal depletion spectrum to maximize the final $P_{FR}$ product yield and minimize the unwanted \pr population.
Figure~\ref{DepWLScan} shows the dependence of the population as the depletion wavelength is scanned from 700-950 nm. The stimulated emission cross-section of both states is higher at shorter wavelengths, increasing the depletion quenching of the excited state, but reducing the selectivity. In addition, at $\lambda_{Dep}<$750 nm the \pfr ground state is also absorbing the depletion pulse at a non-trivial rate, initiating the reverse reaction we are attempting to halt.
At longer wavelength there is an increased difference in the response of the states but lower overall depletion due to the falling cross-section. The maximum effective enhancement of the \pfr state is found between 830 - 840 nm, with the enhanced photoequilibrium of $[P_{FR}]_{EQ}=90.25\%$. Varying the spectral width of the depletion pulse has slightly more effect than varying the excitation spectral width, but again is the same as averaging over the features of the wavelength dependence. Without the use of complex pulse shaping, the depletion spectrum should be kept as narrow as possible while still being broad enough to support the desired temporal pulse characteristics.
This behavior will likely be different with optimally tailored, shaped pulse excitation-depletion. A spectrally broad depletion pulse with a spectral phase designed such that its instantaneous frequency was relatively narrow and followed the dynamically varying energy difference between an excited wavepacket and the ground state should be more effective, but can not be represented by the present model.

\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{ch-OG/Figs/REM/DepWLScan.png}
  \caption[Depletion Wavelength Dependence the Stimulated Depletion Quenching]{Dependence of the SDQ enhanced equilibrium population of the \pr and \pfr states on the depletion wavelength, under fixed excitation power, depletion power, and pulse durations and delays. The optimum depletion wavelength is approximately 833 nm, yielding an enhanced final \pfr population of 90.25\%.}\label{DepWLScan}
\end{figure}

Next we measure the power dependence of the SDQ. The depletion pulse power is varied while the spectrum is fixed at the optimal wavelength of 833 nm with a spectral width of 10 nm, the excitation pulse is 0.20 mW, 30 nm bandwidth centered at 625 nm, with a pulse duration of 100 fs. The depletion pulse duration is 140 fs and the excitation-depletion delay is 0.08 ps. Figure~\ref{DepPowScan} shows the power dependence of the SDQ enhanced populations. Even at low depletion power there is an increase in \pfr over the linear equilibrium of 70\%.
With these exposure parameters the SDQ enhanced \pfr population passes 90\% with a depletion pulse power of 6.5 mW.
Within this model, the enhancement of the \pfr state is likely not to reach 100\% \pfr, as there will always be a residual reverse reaction to produce a trace of \pr. As the depletion power increases the final photoequilibrium is shifted to higher \pfr population, however the higher depletion powers also slow the photoswitching reaction, thereby increasing the number of exposures necessary to reach this higher equilibrium state, as shown in the chart of the $N_{DEC}$ inset in Figure~\ref{DepPowScan}.
%Further, we saw in the single exposure simulations in Section~\ref{Sec:OG:REMSingle} that due to the ultrafast dynamics of the photo-isomerization it is not realistically possible to achieve 100\% depletion of the $P_{FR}$* excited state without also completely depleting the $P_{R}$* excited state, some small population is always able to begin isomerizing.
The maximum \pfr population achievable with a depletion power of 10 mW is 92.5\%; increasing the power to 50 mW this can be increased to 92.7\% (this power is far above the acceptable power range for this model, this would not just cause damage to the molecule but filamentation and dielectric breakdown of the solution).
This remark does not necessarily mean that more sophisticated models or experimental operating conditions which address the ultrafast coherent dynamics of the excited state will not be able to break through this new higher photoequilibrium threshold to come even closer to the 100\% \pfr state.


\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{ch-OG/Figs/REM/DepPowerScan}
  \caption[Power Dependence of the SDQ]{Dependence of the SDQ enhanced equilibrium population on the depletion pulse power; under fixed excitation power, spectrum, duration, and excitation-depletion delay. With these parameters the enhanced \pfr population surpasses 90\% with a depletion power of 6.5 mW. The inset shows that while increasing the power enhances the final equilibrium population, it also increases the decimation count $N_{DEC}$ by slowing the photoswitching reactions in both directions.}\label{DepPowScan}
\end{figure}

Finally we vary the temporal parameters of the depletion pulse. In general, increasing the depletion pulse duration (while maintaining the same instantaneous intensity) should increase the depletion of an excited state; the longer the depletion pulse interacts with the system the higher the probability it will trigger the transition to the ground state by stimulated emission. However, maximizing the depletion of the $P_{FR}^\ast$ state by lengthening the pulse will also lead to increased depletion of the slower to develop $P_{R}^\ast$ state, eliminating the selectivity of the quenching enhancement. The optimal pulse duration and delay will balance these opposing demands, interacting with the system as long as possible while still maintaining a selective enhancement. Beyond that, the gains of quenching the reverse reaction are outweighed by the losses caused by preventing the forward reaction.
To find the optimal depletion delay and pulse duration, these two parameters are scanned in concert at the optimal central wavelength of 833 nm with a depletion power of 6.5 mW. This 2-dimensional scan is shown in Figure~\ref{Fig:OG:Temp2D}. The peak of the surface occurs at a delay of 0.08 ps and pulse duration of 0.14 ps with an equilibrium \pfr population of 90.25\%.

\begin{figure}
  \centering
  \includegraphics[width=.95\linewidth]{ch-OG/Figs/REM/Temporal2Dscan.png}
  \caption[2-D scan of Depletion Temporal Parameters]{\uline{2-D scan of depletion pulse temporal parameters:} Dependence of the \pfr equilibrium population on the excitation-depletion pulse delay and depletion pulse duration. Depletion spectrum is set at the previously determined optimal value of 10 nm at 830 nm central frequency. The peak value of the enhanced \pfr photoequilibrium is 90.35\%  at a delay of 0.08 ps and pulse duration of 0.14 ps.}\label{Fig:OG:Temp2D}
\end{figure}

It is interesting to note that significant quenching enhancement can be achieved with the depletion pulse arriving before the excitation pulse if the width of the depletion pulse is greater than the negative delay. This allows the depletion pulse to interact at high intensity with the excited \pfr state as early as possible, without waiting for the leading edge of the depletion pulse to ramp up. This also helps to have the depletion pulse drop away before the excited \pr state fully develops. At higher power, the pulse can be moved to shorter or more negative delays, as the power on the trailing edge is high enough to overcome wasting the higher peak intensity before the population arrives at the lower level of the electronic excited state. Raising the power to 10 mW increases the equilibrium \pfr population to 92.5\%, but also shifts the optimal depletion pulse to 10 femtoseconds shorter delay and 25 fs longer duration to compensate. At a power of 10 mW it is possible to achieve higher than 90\% \pfr with zero delay pulses.



%\tcr{first calculate the dependence of the final $P_{FR}$ population after 50 iterations on the excitation-depletion delay at a fixed width of 150 fs. These measurements are shown in Figure~\ref{DelayScan}. The depletion spectrum is centered at 835 nm; all other laser parameters are listed in Table~\ref{Table:OG:LaserParam}. The excitation depletion delay is varied from 0.05 - 0.25 ps with the optimum delay between 0.15-0.16 ps, which is approximately equal to the calculated peak of the dynamic population of the $P_{FR}$* FR3 level. This shows that the best depletion pulse arrival time would be as soon as the relaxation from the Frank-Condon initial excitation point on the potential energy surface has completed and before the molecule has completed further progress toward the isomerization branching point on the excited state surface.}

%\begin{figure}
%  \centering
%  \includegraphics[width=.8\linewidth]{ch-OG/Figs/Exp/DelayScan}
%  \caption[Excitation-Depletion Delay dependence of Quenching]{Dependence of the final relative concentration of the $P_{FR}$ state on the excitation-depletion delay, under fixed excitation power, depletion power, pulse durations and spectra. The optimum delay is approximately 150 fs.}\label{DelayScan}
%\end{figure}
%
%Finally we vary the depletion pulse duration at the previously determined optimum wavelength (840 nm) and depletion delay (0.155 ps) to maximize the interaction time and determine the optimal excitation-depletion pulse characteristics. This is shown in Figure~\ref{Fig:OG:WidthScan}. The $P_{FR}$ population initially rises due to increased depletion quenching, peaks at an optimal duration of approximately 150 fs, and gradually falls as the depletion of the $P_{R}$* excited state begins to undermine the quenching enhancement of the reverse direction by quenching the forward reaction.
%
%\begin{figure}
%  \centering
%  \includegraphics[width=.8\linewidth]{ch-OG/Figs/Exp/WidthScan}
%  \caption[Depletion Pulse Duration dependence of Quenching]{Dependence of the final relative concentration of the $P_{FR}$ state on the depletion pulse duration, under fixed excitation power, depletion power, and pulse spectra. Two sets of data are shown at different excitation-depletion delays: the optimum delay of 0.150 ps (blue diamonds), and the synchronized excitation and depletion pulses at 0.0 ps (red squares). The optimum depletion pulse duration is approximately 150 fs at the optimum delay of 0.150 ps.}\label{Fig:OG:WidthScan}
%\end{figure}
%



%
%
%
%% ======================================================================================================================
%% ======================================================================================================================

%% ##################################################################################
% Done Here! On to Next Section! 

==> main.tex <==
\RequirePackage{import}
\import{paper/}{ch-OG/Figs/REM/1.tex}
